Improved Submodular Secretary Problem with Shortlists

First, for the for the submodular $k$-secretary problem with shortlists [1], we provide a near optimal $1-1/e-\epsilon$ approximation using shortlist of size $O(k poly(1/\epsilon))$. In particular, we improve the size of shortlist used in \cite{us} from $O(k 2^{poly(1/\epsilon)})$ to $O(k poly(1/\epsilon))$. As a result, we provide a near optimal approximation algorithm for random-order streaming of monotone submodular functions under cardinality constraints, using memory $O(k poly(1/\epsilon))$. It exponentially improves the running time and memory of \cite{us} in terms of $1/\epsilon$. Next we generalize the problem to matroid constraints, which we refer to as submodular matroid secretary problem with shortlists. It is a variant of the \textit{matroid secretary problem} \cite{feldman2014simple}, in which the algorithm is allowed to have a shortlist. We design an algorithm that achieves a $\frac{1}{2}(1-1/e^2 -\epsilon)$ competitive ratio for any constant $\epsilon>0$, using a shortlist of size $O(k poly(\frac{1}{\epsilon}))$. Moreover, we generalize our results to the case of $p$-matchoid constraints and give a $\frac{1}{p+1}(1-1/e^{p+1}-\epsilon )$ approximation using shortlist of size $O(k poly(\frac{1}{\epsilon}))$. It asymptotically approaches the best known offline guarantee $\frac{1}{p+1}$ [22]. Furthermore, we show that our algorithms can be implemented in the streaming setting using $O(k poly(\frac{1}{\epsilon}))$ memory.

==> Impossiblesave.tex <==
%\section{Impossibility Result}

In this section we provide an upper bound showing the following:

\hardness*

%\begin{theorem}
%There is no algorithm achieving asymptotic competitive ratio $7/8+\epsilon$ for submodular secretary problem using $o(n)$ selections. 
%\end{theorem}

%\mcomment{In the following proof we will consider a submodular $k+1$-secretary} problem. 
In the following proof, for simplicity of notation, we prove the desired bound for submodular $k+1$-secretary problem. %Since $k+1=O(k)$, the upper bound derived will imply the stated bound for the  submodular $k$-secretary problem. 
First, we define a monotone submodular function $f$ as follows. 
For $n>0$, the ground set consists of two types of elements, $A$ and  $B$, such that
$f(a)=k$ for $a\in A$ and $f(b)=1$ for $b\in B$. %There are infinitely many elements of $A$ and $B$. 
\scomment{Don't you just need $L$ items of type $A$ and $n-1$ items of type $B$?}
There are $L:=n/2k$ items of type $A$ and
$n-1$ items of type $B$.
Also there is a collection of {\it disjoint} sets $T_{\ell}=\{a_1^{\ell}, b_1^{\ell},\cdots, b^{\ell}_{k}\}$, $\ell=1,2, \ldots L$, such that $a_1^{\ell}\in A$ and $b_j^{\ell}\in B$, and $f(T_{\ell})=2k$.
\scomment{infinite number of such sets? or will $L$ suffice?} 
\mcomment{in the definition of function it should be infinite but in the input we use $n/2k$ of them}
\scomment{After going through the proof, I don't see why you need infinite number, it seems just $L=n/2k$ will suffice. Where are you using that there are infinte number of $T^\ell$?}
\mcomment{
The reason is that you should give one functions $f$ that works for all $n$. Otherwise one may claim that for any given function $f$ there is large enough $N_f$ so that we can go beyond 7/8, for $n>N_f$. 
}

Now define 
$$g(t):=k+k/2+\cdots+ (t-ik)/2^i$$
where $i=\floor{t/k}$. It is easy to see that $g$ is a monotone submodular function.
Now define $f$ as follows:
\begin{itemize}
\item $|S\cap A| \ge 2 \implies f(S):=2k+1$
\item $|S\cap A|=0 \implies f(S):=1+g(|S|-1)$
\item $|S\cap A|=1 :$
\begin{itemize}
\item $S\cap A\notin\{a^{\ell}_1\}_{\ell>0} \implies f(S):=k+\frac{1}{2} g(|S|-1)$
\item $S\cap A= \{a_1^{\ell}\}$ for some $\ell$  $\implies f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+k'/2^{i+1}\}$, where $k'=|S\cap\{b^{\ell}_1,\cdots, b_k^{\ell}\} |$.
\end{itemize}
\end{itemize}
Note that for any subset $S$, $f(S)\le 2k+1$.
\begin{lemma}
$f$ is a monotone submodular function.
\end{lemma}
\begin{proof}
We have to show that for elements $x$ and subsets $S\subseteq T$, $\Delta_f(x|S) \ge \Delta_f(x|T)$.
We consider the following cases:
\begin{itemize}
\item if $|T\cap A| \ge 2 \implies f_T(x)=0$, so it is trivial.
\item if $|T\cap A| =0 \implies |S\cap A|=0 \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\item if $|T\cap A|=1 \implies |S\cap A|\le 1$
\begin{itemize}
\item if $|S\cap A|=1 :$
\begin{itemize}
\item $S\cap A = T\cap A = \{a_1^{\ell}\}:$
\begin{itemize}
\item $x\in \{b_1^{\ell},\cdots, b_k^{\ell}\} \implies \Delta_f(x|S)=1/2^i+1/2^i$ and $\Delta_f(x|T)=1/2^j+1/2^j$ for $j\ge i$.
\item $x\notin \{b_1^{\ell},\cdots, b_k^{\ell}\} \implies \Delta_f(x|S)=1/2^i$ and $\Delta_f(x|T)=1/2^j$ for $j\ge i$.
\end{itemize}
\item $S\cap A = T\cap A \notin \{a_1^{\ell}\}_{\ell} \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\end{itemize}
\item if $|S\cap A|=0 \implies \Delta_f(x|T) \le 1/2^{i+1}+1/2^{i+1}$ and $\Delta_f(x|S)= 1/2^j$ for $j\le i$. Thus $\Delta_f(x|S) \ge \Delta_f(x|T)$.
\end{itemize}
\end{itemize} 
Monotonicity is trivial.
\end{proof}

\toRemove{
Also for any subset of $S$ with at least two elements of $A$, $f(S)=2k$. 
For subset $S$ with no element in $A$, if $i=\floor*{\frac{|S|}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+k/2+ \dots +(|S|-ik)/2^{i}.
\]
For subset $S$ with exactly one element $a\in A$ such that $a\neq a_1$, if if $i=\floor*{\frac{|S|-1}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+ k/2+ \dots +(|S|-1-ik)/2^{i+1}.
\]
Thus if $|S|=k+1$ and it contains exactly one element of $a\in A$ such that $a\neq a_1$ then $f(S)=k+k/2$.
Now suppose $S$  contains $a'$. 
For $S=T$, $f(S)=2k$.  Suppose $S$ contains $k'<k$ elements of $\{b_1, \dots, b_k\}$  and $\ell$ other elements of $B$. 
Let's $t=k'+\ell$, and $i=\floor*{\frac{t}{k}}$, then
\[
f(S)= \min\{2k, k'/2+(k+ k/2+ \dots +(t-ik)/2^{i+1})\}
\]
}
%\scomment{this proof is very vague, especially the claim any algorithm will select $k/2$ of $B$? Phrases like algorithm is not "aware" of something cannot be stated as a fact. You need to prove that the algorithm will not be able to distinguish between the two scenarios. We need to discuss.}



%Let $ {\cal T}^L$ be a collection of (any) $L=n/2k$ sets from $T^\ell, \ell=1,2, \ldots$. W.l.o.g., let's assume ${\cal T}^\ell = \{T_1, \ldots, T_L\}$.   

Denote $B^{\ell} := T^\ell \cap B = \{b_1^{\ell},\cdots, b_k^{\ell}\}$ for $\ell=1,2, \ldots,$. Also, let 
$B'=B\setminus (\bigcup_{\ell=1}^L B^{\ell})$. % where $L:=n/2k$. 
%\scomment{Do you need $T^\ell, \ell =1,\ldots, L$ to be disjoint?} \mcomment{yes}
% $B'=B\setminus (\bigcup_{\ell }^{L} B^{\ell})$ for $L:=n/2k$.
Now define $L$ input instances $\{I_{\ell}\}_{\ell =1,\ldots, L}$, each of size $n$, as follows. For
any arbitrary subset $\tilde{B}\subseteq B'$ of size $n-Lk-1$, 
%\scomment{Which subset $\tilde{B}$? any arbitrary subset?} \mcomment{arbitrary}
define $I_{i}=\bigcup_{\ell=1,\ldots, L}  B^{\ell} \cup \tilde{B} \cup \{a_1^{i}\}$, for  $i=1,\ldots, L$.
%and $I_2=B^1 \cup B^2 \cup \tilde{B} \cup \{a_1^2\}$ (the difference is $a_1^1$ and $a_1^2$).
%Now suppose the input consists of the following:  $T^{\ell}=\{a_1^{\ell}, b_1^{\ell}, \cdots b_k^{\ell} \}$, no other element of $A$ and the remaining elements are from $B':=B\setminus \{b_1^{\ell}, \cdots, b_k^{\ell}\}$. 
Thus the optimal is $T^{\ell}$ for instance $I_{\ell}$, with $f(T^{\ell})=2k$. 
\scomment{$T^\ell$ is of size $k+1$, optimal should be of size $k$. If making $T_\ell$ to be of size $k$ makes it messy, you can initially state that you will consider submodular $k+1$ secretary problem.}


Now consider any algorithm for the submodular \nameSecSL~,and cardinality constraint $k+1$. We denote by $Alg$ the set of $\eta(k+1)$ items selected by the algorithm as part of the shortlist. % (all elements in the shortlist of size $\eta(k)$).
\scomment{We have  used $A$ to denote shortlist in the algorithm. May be you can use a different symbol instead of type $A$ and $B$. }
Let $\bar I$ denote an instance chosen uniformly at random from $I_\ell, \ell=1,\ldots, L$.  
%We choose one of $I_{\ell}$ randomly. \scomment{randomly or arbitrarily?} 
Let $\pi$ denote a random ordering of $n$ items in $\bar I$. 
%We give a random order of $I_{\ell}$, say $\pi$ to the algorithm as input,
%(note that in the secretary problem the elements of input can be selected adversarially but the order should be random).
We denote by random variable $(\bar{I},\pi)$ the randomly ordered input instance to the algorithm. Also we denote by $\bar{T}, \bar{B}$ and $\bar a$, the corresponding $T^{\ell}$, $B^{\ell}$ and $a_1^\ell$.

Now we claim 

%Note that algorithm is not aware of $\ell$.
%Consider an algorithm $Alg$.
%Suppose $a_1^{\ell}$ is the $t$-th elements in the input, and
%elements of input are ordered as $I=(I_1,\cdots, I_n)$.
%Suppose $Alg$ is the set of elements selected by an algorithm.
%Denote by $\bar{B}=\{b_1,\cdots, b_k\}$.

\begin{lemma}
$\mathbb{E}_{(\bar{I},\pi)}[|Alg\cap \bar{B}|] \le k/2+\eta(k+1)/L$.
\end{lemma}
\begin{proof}
Suppose $(e_1,\cdots, e_n)$ indicates the ordered input according to random ordering $\pi$ on $\bar{I}$. %for some $0<\ell<L$.
Now let $t$ be the random variable indicating the index of $a_1^{\ell}$ in $(e_1,\cdots, e_n)$, i.e., $e_t=a_1^{\ell}$. 
%Define $R:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}|]$.
Then, due to random ordering, and random choice of $\bar I$ from $I_1, \ldots, I_\ell$, we have
$$\mathbb{E}_{(\bar I, \pi)}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^1|]= \cdots = \mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap B^{L}|]\ .$$
Also, since $B^\ell, \ell=1,\ldots, L$ are disjoint,
$$\sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^{\ell}|] \le \eta(k+1)\ .$$
Since $\bar B=B^\ell$ with probability $1/L$,  we have
$$H:=\mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap \bar{B}|]=  \frac{1}{L} \sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap B^{\ell}|] \le \frac{1}{L} \eta(k+1)\ . $$ 
%\rightarrow 0$ as $n/\eta(k) \rightarrow \infty$.
Now define
$G:=\mathbb{E}[|Alg\cap\{e_t,\cdots, e_{n}\}\cap \bar{B}|]$.
We have
$$G\le \mathbb{E} [|\bar{B}\cap\{e_t,\cdots, e_n\}|]  \le k/2\ .$$
%Also define $H:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\cap \bar{B}\}|]$.
%Also, $H\le k-G$.
Thus $$\mathbb{E}[|Alg\cap \bar{B}|] \le G+H\le k/2+\eta(k+1)/L\ .$$
%\rightarrow G$$
%\le k/2$$
%G+(k-G)/2 \le k/2+G/2\le k/2+k/4=3/4k$$.
\end{proof}
Now on input $\bar{I}$, if the algorithm doesn't select $\bar a$, then $f(Alg)\le k+k/2$. Otherwise, if algorithm selects $\bar a$ then 
$$f(Alg)= k+ \frac{1}{2} g(k)+\frac{1}{2} |Alg\cap \bar{B}|$$ therefore $$\mathbb{E}[f(Alg)] \le k+\frac k 2+ \frac k 4+ \frac{\eta(k+1)}{2L} = \frac{7k}{4} + \frac{k\eta(k+1)}{n} \ .$$
%Hence $\mathbb{E}[f(Alg)]  \rightarrow k+k/2+k/4$ as $n\rightarrow \infty$, since $\eta(k)=o(n)$.
Since the optimal is at least $\Ex[f(\bar T)]=2k$, the competitive ratio is upper bounded by
$$ 
%\left(\frac{7k}{4} + \frac{k\eta(k)}{n}\right)\left/\right. 2k = 
\frac{7}{8} + \frac{\eta(k+1)}{2n} = \frac{7}{8} + o(1)\ ,$$
where we used $\eta(k+1)=o(n)$.
\scomment{I think we need to change the upper bound in theorem statement to $7/8 + o(1)$}
%Before arriving $a_1^{\ell}$ algorithm can not distinguish between elements of $B'=\{b_1^{\ell},\dots, b_k^{\ell}\}$
%and the rest of $B$ thus the expected number of elements in $B'$ selected by algorithm before observing $a_1$ goes to $0$ as $n/k\rightarrow \infty$.

%Therefore an online algorithm would select $k/2$ elements of set $B'$ in expectation and also it selects $a_1^{\ell}$ (and $k/2$ other elements from $B\setminus B'$).  Therefore, its $f$ value is $k+k/2+k/4$.
%Hence the competitive ratio is at most $7/8$.


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> algorithms1.tex <==
%\section{Algorithms}
%\subsection{Simpler but unimplementable, offline version}
%\subsection{Algorithm description}

Before giving our algorithm for \nameOfProblemSL, we describe a simple technique for \nameSecSL~
that achieves a  $1-\delta$ competitive ratio for  with shortlists of size logarithmic in $1/\delta$.
Recall that in the \nameSec, the aim is to select an item with expected value close to the maximum among a pool of items $I=(a_1, \ldots, a_N)$ arriving sequentially in a uniformly random order. 
We will consider the variant with shortlists, where we now want to pick a shortlist which contains an item with expected value close to the maximum.
%\ccomment{why are we using $\epsilon$ in the text and $\delta$ in the Algorithm below}\scomment{fixed}
We propose the following simple algorithm. For the first $n\delta/2$ rounds, don't add any items to the shortlist, but just keep track of the maximum value seen so far.
For all subsequent rounds, 
for any arriving item $i$ that has a value $a_i$ greater than or equal to the maximum value seen so far, add it to the shortlist if the size of shortlist is less than or equal to $L=4\ln(2/\delta)$. This algorithm is summarized as Algorithm \ref{alg:SIIImax}. Clearly, for contant $\delta$, this algorithm uses a shortlist of size $L=O(1)$. Further, under a uniform random ordering of input, we can show that the maximum value item will be part of the shortlist with probability $1-\delta$. (See Proposition \ref{maxanalysis} in Section \ref{sec:analysis}.)
%that the expected number of items in the shortlist $A$ is at most $\log(1/\epsilon)$, i.e., $O(1)$, and the maximum value item will be part of the shortlist with probability $1-\epsilon$. %analysis is presented in Section \ref{sec:max}. 
%--------------------------------------
\begin{algorithm*}[ht]
  %\caption{~\bf{Select-If-it-Improves}($I , u$)}
  \caption{~\bf{Algorithm for secretary with shortlist} (finding max online)}
  \label{alg:SIIImax} 
\begin{algorithmic}[1]
\State Inputs: number of items $N$, items in $I=\{a_1, \ldots, a_N\}$ arriving sequentially, $\delta \in (0,1]$. 
\State Initialize: $A\leftarrow \emptyset$,  $u=n\delta/2$, $M = -\infty$ %$M\leftarrow \max\{a_1, \cdots, a_{u-1}\}$
%\scomment{Should initialization of $u$ be changed to $n\delta/2$?}
%\mcomment{yes}
\State $L \leftarrow 4\ln(2/\delta)$ %\scomment{I changed (3+$\sqrt{2}$) to $4$}

\For {$i= 1$ to $N$}
%\If {$F(S\cup \{a_i\}) > F(S) $}
\If {$ a_i > M$}
\State $M \leftarrow  a_i$
\If {$i \geq u$ and $|A|<L$}
\State $A\leftarrow A\cup \{a_i\}$
\EndIf
\EndIf
\EndFor
%\State return $S\setminus \{a_1,\cdots, a_u\}$

%\mcomment{
%cleaner:
%\For {$i= u$ to $N$}
%\If {$ a_i > \max_{1\le j <i} a_j$ and $|A|<L$}
%\State $A\leftarrow A\cup \{a_i\}$
%\EndIf
%\EndFor
%}

\State return $A$, and $A^*:= \max_{i\in A} a_i$
\end{algorithmic}
\end{algorithm*}
%--------------------------------------------

%-----------------------------------------
\begin{algorithm*}[h!]
  %\caption{~\bf{Select-If-it-Improves}($I , u$)}
  \caption{~\bf{Algorithm for {\bf submodular} $k$-secretary with shortlist}}
  \label{alg:main} 
  \label{alg:tmp} 
\begin{algorithmic}[1]
\State Inputs: set $\bar I=\{\bar{a}_1,\ldots, \bar{a}_n\}$ of $n$ items arriving sequentially, submodular function $f$, parameter $\epsilon \in (0,1]$. 
\State Initialize: $S_0 \leftarrow \emptyset, R_0 \leftarrow \emptyset, A \leftarrow \emptyset, A^* \leftarrow \emptyset$, constants $\alpha \ge 1, \beta \ge 1$ which depend on the constant $\epsilon$.
\State Divide indices $\{1,\ldots, n\}$ into $(\alpha, \beta)$ windows as prescribed by Definition \ref{def:windows}.
%Divide the sequence of candidates into consecutive groups of $\frac{n}{\beta k}$ candidates, referred to as slots (or buckets). And, divide the sequence of slots into consecutive groups of $\alpha \beta$ slots, referred to as {\it windows}.
%===========================
\For {window $w= 1, \ldots, k/\alpha$} 
%\State For every $\alpha$-length subsequence $\tau=(s_1,\ldots, s_\alpha) \subseteq [\alpha\beta]$ of slots in window $w$, define 
%$$\gamma(\tau):=\{i_1, \ldots, i_\alpha\}$$
%where 
%$$i_j := \arg \max_{i\in V_{s_j,w} \cup R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\})$$
%\State Define $R_w:=\{\cup_{\tau} \gamma(\tau)\}.$ 
 

%\State Process the online inputs in window $w$ using the subroutine in Algorithm \ref{alg:tmpWindow} to select a subset $H_w$ of items. 
 \For {every slot $s_j$ in window $w$, $j=1,\ldots, \alpha\beta$}
  \State Concurrently for all subsequences of previous slots $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ of length $|\tau|<\alpha$ \label{li:subb}   \hspace{0.44in} in window $w$, call the online algorithm in Algorithm \ref{alg:SIIImax} with the following inputs: 
  %\begin{center}
  \begin{itemize}[leftmargin=0.7in]
  \item   number of items $N=|s_j|+1$, $\delta=\frac{\epsilon}{2}$, and
%  \scomment{You have to use $\delta$ smaller than $\epsilon$ to get $1-\frac{1}{e}-\epsilon$ in the final result.}
  \item item values $I=(a_0, a_1, \ldots, a_{N-1})$, with 
     \begin{eqnarray*} 
  a_0 & := & \max_{x\in R_{1,\ldots, w-1}} \Delta(x|S_{1,\ldots,w-1} \cup \gamma(\tau)) \\
  %\max_{x\in R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{x\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\}$
     a_\ell & := & \Delta(s_j(\ell)| S_{1,\ldots,w-1} \cup \gamma(\tau) ),  \forall \ell=1,\ldots, N-1
     \end{eqnarray*}
    %f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$
 where $s_j(\ell)$ denotes the $\ell^{th}$ item in the slot $s_j$. 
% \item $\delta = \frac{\epsilon}{{\alpha \beta \choose \alpha}}$.
  \end{itemize}
   %\end{center}
   %\mcomment{why do you divide by... the erros do not add up}  \scomment{Please add the required theorem showing this}  \mcomment{added lemma~\ref{online}}
\State Let $A_{j}(\tau)$ be the shortlist returned by  Algorithm \ref{alg:SIIImax} for slot $j$ and subsequence $\tau$. Add 
\label{li:tmp} \hspace{0.44in} all items except the dummy item $0$ to the shortlist $A$. Let's $A(j)=\bigcup_{\tau} A_j(\tau)$.
%for all $\tau$,
%  $$A(j) \leftarrow A(j)\cup (A_{j}(\tau))$$
%$H_w$, i.e, for all $\tau$,
 % $$H_w \leftarrow H_w\cup (A_{j}(\tau) \cap s_j)$$
 That is, \label{li:sube}
 $$A\leftarrow A\cup  (A(j)\cap s_j)$$
 \EndFor
%\State return $H_w$
% \State $A\leftarrow A\cup H_w$
 \State \label{li:Rw} After seeing all items in window $w$, compute $R_w, S_w$ as defined in \eqref{eq:Rw} and \eqref{eq:Sw} respectively.
 \State $A^* \leftarrow A^*\cup (S_w \cap A)$
\EndFor
\State return $A$, $A^*$. %$A=T_1 \cup \cdots  \cup T_{W}$
\end{algorithmic}
\end{algorithm*}

%==========================


%\begin{algorithm*}[ht]
  %\caption{~\bf{Subroutine of Algorithm \ref{alg:tmp} for window $w$}}
  %\label{alg:tmpWindow} 
  \toRemove{
  \begin{algorithmic}[1]
  \For {every slot $s_j$ in window $w$, $j=1,\ldots, \alpha\beta$}
  \State Concurrently for all subsequences of previous slots $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ in window $w$, of length $|\tau|<\alpha$, call the online algorithm in Algorithm \ref{alg:SIIImax} with the following inputs: number of items $N=|s_j|+1$, $\delta = \frac{\epsilon}{{\alpha \beta \choose \alpha}}$, \mcomment{why do you divide by... the errors do not add up} and values of arriving items $(a_0, a_1, \ldots, a_{N-1})$ defined as 
  $$a_0:=\max_{x\in R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{x\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\}$$
    $$a_i :=f(S_{1,\ldots,w-1} \cup \gamma(\tau) \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$$
 where $i$ denotes the $i^{th}$ item in slot $s_j$.
  \State Let $A_{j}(\tau)$ be the shortlist returned by  Algorithm \ref{alg:SIIImax} for slot $j$ and subsequence $\tau$. Add all items except the dummy item $0$ to $H_w$, i.e, for all $\tau$,
  $$H_w \leftarrow H_w\cup (A_{j}(\tau) \cap s_j)$$
 \EndFor
\State return $H_w$
\end{algorithmic}
}
%\end{algorithm*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
There are two main difficulties in extending this idea to the \nameOfProblemSL. First, instead of one item, here we aim to select a set $S$ of $k$ items using an $O(k)$ length shortlist. Second, the contribution of each new item $i$ to the objective value, as given by the submodular function $f$, depends on the set of items selected so far. 

The first main concept we introduce to handle these difficulties  is that of dividing the input into sequential blocks that we refer to as $(\alpha, \beta)$ windows. Below is the precise construction of $(\alpha, \beta)$ windows, for any postivie integers $\alpha$ and $\beta$, such that $k/\alpha$ is an integer.
%\ccomment{This definition is imprecise.  Needs to be made technically crisp.}
%\ccomment{What exactly is this distribution?  Are we drawing with replacement or without and do the $X_i$ sum to $n$?}

We use a set of random variables $X_1,\ldots,X_m$ defined in the following way.  Throw $n$ balls into $m$ bins uniformly at random.  Then set $X_j$ to be the number of balls in the $j$th bin.  We call the resulting $X_j$'s a {\em $(n,m)$-ball-bin random set}.


\begin{definition}[$(\alpha,\beta)$ windows]
\label{def:windows}
Let $X_1,\ldots,X_{k\beta}$ be a $(n,k\beta)$-ball-bin random set.
Divide the indices $\{1,\ldots, n\}$ into $k\beta$ slots, where the $j$-th slot, $s_j$, consists of $X_j$ consecutive indices in the natural way, that is, slot $1$ contains the first $X_1$ indices, slot $2$ contains the next $X_2$, etc.
 %, $X_i$ would be the number of balls in the $i$-th bin.
 Next, we define $k/\alpha$ windows, where window $i$ consists of $\alpha \beta$ consecutive slots, in the same manner as we assigned slots.
\end{definition}
%\ccomment{Would an example or a figure help here to define slots and windows?}
Thus, $q^{th}$ slot is composed of indices $\{\ell, \ldots, r\}$, where $\ell=X_1+...+X_{q-1}+1$ and  $r=X_1+...+X_q$. 
Further, if the ordered the input is $\bar a_1, \dots, \bar a_n$ then we say that the items inside the slot $s_q$ are $\bar a_{\ell}, \bar a_{\ell+1}, \dots, \bar a_{r}$ 
To reduce notation, when clear from context, we will use $s_q$ and $w$ to also indicate the {\it set of items} in the slot $s_q$ and window $w$ respectively.

%The idea is to divide the inputs into $k/\alpha$ blocks (i.e., windows) for a constant $\alpha\ge 1$ such that 
%\ccomment{Shouldn't we say what alpha is because the intuition depends on it}
When $\alpha$ and $\beta$ are large enough constants, some useful properties can be obtained from the construction of these windows and slots. First, roughly $\alpha$ items from the optimal set $S^*$ are likely to lie in each of these windows; and further, it is unlikely that two items from $S^*$ will appear in the same slot. (These statements will be made more precise in the analysis where precise setting of $\alpha,\beta$ in terms of $\epsilon$ will be provided.) Consequently, our algorithm can focus on identifying a constant number (roughly $\alpha$) of optimal items from each of these windows, with at most one item coming from each of the $\alpha \beta$ slots in a window. The core of our algorithm is a subroutine that accomplishes this task in an online manner using a shortlist of constant size in each window. 

To implement this idea, we use a greedy selection method that considers all possible $\alpha$ sized subsequences of the $\alpha\beta$ slots in a window, and aims to identify the subsequence that maximizes the increment over the best items identified so far. 
More precisely, for any subsequence $\tau=(s_1,\ldots, s_\ell)$ of the $\alpha\beta$ slots in window $w$, we define a `greedy' subsequence $\gamma(\tau)$ of items as:
\begin{equation}
\label{eq:gamma}
\gamma(\tau):=\{i_1, \ldots, i_\ell\}
\end{equation}
where
\begin{equation}
\label{eq:ij}
i_j := \arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} f(S_{1, \ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1, \ldots, w-1} \cup \{i_1\ldots, i_{j-1}\}).
\end{equation}
In ({\ref{eq:ij}) and in the rest of the paper, we use shorthand $S_{1,\ldots, w}$ to denote $S_1\cup \cdots \cup S_{w}$, and $R_{1,\ldots, w}$ to denote $R_1\cup \cdots \cup R_{w}$, etc.  We also will take unions of subsequences, which we interpret as the union of the elements in the subsequences.
%\ccomment{Are we bothered by taking the union of a sequence rather than a set?}
We also define $R_w$ to be  the union of all greedy subsequences of length $\alpha$, and $S_w$to be  the best subsequence among those. That is,
\begin{equation}
\label{eq:Rw}
R_w = \cup_{\tau: |\tau|=\alpha} \gamma(\tau)
\end{equation}
and 
\begin{equation}
\label{eq:Sw}
S_w=\gamma(\tau^*),
\end{equation} where
\begin{equation}
\label{eq:taustar}
\tau^*:=\arg \max_{\tau: |\tau|=\alpha} f(S_{1,\ldots,w-1} \cup \gamma(\tau)) - f(S_{1,\ldots,w-1}).
\end{equation}
Note that $i_j$ (refer to \eqref{eq:ij}) can be set as  either an item in slot $s_j$ or an item {\it from a previous greedy subsequence} in $R_1\cup \cdots \cup R_{w-1}$. The significance of the latter relaxation will become clear in the analysis.
%Here, $s_j \cup R_1 \cup \cdots \cup R_{w-1}$ denotes the union of items in slot $s_j$ and 

%$S_w$ represents the best subsequence among all the subsequences in $R_w$.
As such, identifying the sets $R_w$ and $S_w$ involves looking forward in a slot $s_j$ to find the best item (according to the given criterion in \eqref{eq:ij}) among all the items in the slot. To obtain an online implementation of this procedure, we use an online subroutine that employs the algorithm (Algorithm \ref{alg:SIIImax}) for the basic secretary problem described earlier. This online procedure will result in selection of a set $H_w$ potentially larger than $R_w$, while ensuring that each element from $R_w$ is part of $H_w$ with a high probability $1-\delta$ at the cost of adding extra $\log(1/\delta)$ items to the shortlist. Note that $R_w$ and $S_w$ can be computed {\it exactly at the end} of window $w$. 

Algorithm \ref{alg:tmp} summarizes the overall structure of our algorithm. 
%The  following notation is used for brevity. For any collection of sets $V_1, \ldots, V_\ell$, we use $V_{1,\ldots, \ell}$ to denote $V_1 \cup \cdots \cup V_\ell$. 
In the algorithm, for any item $i$ and set $V $, we define $\Delta_f(i|V):=f(V\cup \{i\})- f(V)$.
%The subroutine to compute $H_w$ for window $w$ uses Algorithm \ref{alg:SIImax} for each subsequence $\tau$ and each slot $s_j$ in that subsequence. Consequently, the parameters for Algorithm \ref{alg:SIImax} for slot $j$ are: number of items $X_j$ which is $n/k\beta$ in expectation, $\delta >0$, and value $a_i$ of an item $i\in [X_j]$ is as given by the expression inside maximizer in \eqref{eq:ij}.
%\scomment{I will come back to make this more precise with parameter specifications, after finishing the subroutine description and analysis.}

The algorithm returns both the shortlist $A$ which we show to be  of size $O(k)$ in the following proposition, as well as a set $A^*=\cup_w (S_w \cap A)$ of size at most $k$ to compete with $S^*$. In the next section, we will show that $\Ex[f(A^*)] \ge (1-\frac{1}{e} - \epsilon -O(\frac{1}{k})) f(S^*)$ to provide a bound on the competitive ratio of this algorithm. 

\begin{prop}
\label{prop:size}
Given $k,n$, and any constant $\alpha, \beta$ and $\epsilon$, the size of shortlist $A$ selected by Algorithm~\ref{alg:main} is at most $4k \beta {\alpha \beta \choose \alpha}\log(2/\epsilon) = O(k)$. 
%\scomment{proposition about size of shortlist returned by Algorithm \ref{alg:tmp}.}
\end{prop}
\begin{proof}
For each window $w=1,\ldots, k/\alpha$, and for each of the $\alpha\beta$ slots in this window, lines \ref{li:subb} through \ref{li:sube} in  Algorithm \ref{alg:main} runs  Algorithm \ref{alg:SIIImax} for ${\alpha \beta \choose \alpha}$ times (for all $\alpha$ length subsequences). By construction of  Algorithm \ref{alg:SIIImax}, for each run it will add at most $L\le 4\log(2/\epsilon)$ items each time to the shortlist. 
%\scomment{Here, we need to fix what $ \delta$ is in terms of $\epsilon$. I have waiting for your precise theorem about this.} \mcomment{lemma~\ref{online}}
Therefore, over all windows, Algorithm \ref{alg:main} adds at most $ \frac{k}{\alpha} \times \alpha\beta  {\alpha \beta \choose \alpha} L = O(k)$ items to  the shortlist. 
\end{proof}
%Later, in the proof of Theorem \ref{opttheorem}, we show that we set $\alpha=O(\frac{1}{\epsilon^4}\log(1/\epsilon)), \beta=O(\frac{1}{\epsilon^2})$ to get the desired competitive ratio. This setting of $\alpha, \beta$ results in the specific dependence of function $\eta_\epsilon(k)$ on $\epsilon$, as  stated in Theorem \ref{opttheorem}.
%\scomment{Add some sentences regarding the changes in implementation required for the streaming version.}


%\subsection{Preliminary: Algorithm for finding max online}
%Add details about online Algorithm for picking $\log(1/\delta)$ items from a sequence of $n$ items such that max lies in the picked items with probability $1-\delta$.
%Consider the simple greedy algorithm described in algorithm~\ref{alg:SIIImax}.

%\begin{algorithm*}[ht]
%  \caption{~\bf{Select-If-it-Improves}($I , u$)}
%  \label{alg:SIII} 
%\begin{algorithmic}[1]
%\State $S\leftarrow \emptyset$
%\For {i=0 to n}
%%\If {$\max(S\cup \{a_i\}) > \max(S) $}
%\If {$F(a_i) > \max_{a\in S} F(a) $}
%\State $S\leftarrow S\cup \{a_i\}$
%\EndIf
%\EndFor
%\State return $S\setminus \{a_1,\cdots, a_u\}$
%\end{algorithmic}
%\end{algorithm*}




%\begin{theorem}
%Suppose $S$ is the output of above algorithm on the input $I=\{a_1,\cdots, a_n\}$ then $F(S) = F(I)$
%\end{theorem}
%\begin{proof}

%%Suppose $F(I)=f(T)$,  where $|T|=m$. The above algorithm never miss  any element of $T$.
%%Since $F$ is submodular if the marginal increae

%Suppose $S_i$ is the subset selected at iteration $i$. Since $F$ is submodular, if $F(S_i\cup \{a_i\}) \le F(S_i)$ 
%then $F(S\cup\{a_i\}) \le F(S)$. Therefore every $e\in I\setminus S$ has marginal value 0 with respect to $S$, i.e., $F(S)=F(I)$.
%\end{proof}

%\paragraph{Bounds on size of shortlist maintained by Algorithm \ref{alg:tmp}.}



==> bib.tex <==
@misc{shadravan2020submodular,
    title={Submodular Matroid Secretary Problem with Shortlists},
    author={Mohammad Shadravan},
    year={2020},
    eprint={2001.00894},
    archivePrefix={arXiv},
    primaryClass={cs.DS}
}


@misc{kazemi2019submodular,
    title={Submodular Streaming in All its Glory: Tight Approximation, Minimum Memory and Low Adaptive Complexity},
    author={Ehsan Kazemi and Marko Mitrovic and Morteza Zadimoghaddam and Silvio Lattanzi and Amin Karbasi},
    year={2019},
    eprint={1905.00948},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}
\bibitem{kleinberg} R. Kleinberg, A Multiple-Choice Secretary Algorithm with Applications to Online Auctions
\bibitem{vondrak} V. Feldman, J. Vondrak, Optimal Bounds on Approximation of Submodular and XOS Functions by Juntas
\bibitem{kleh} T. Kesselheim, A. Tönnis, Submodular Secretary Problems: Cardinality, Matching, and Linear Constraints
\bibitem{mirzasoleiman} A. Badanidiyuru, B. Mirzasoleiman, A. Karbasi, A. Krause, Streaming Submodular Maximization: Massive Data Summarization on the Fly
\bibitem{bateni} M. Bateni, M. Hajiaghayi, M, Zadimoghaddam,  Submodular Secretary Problem and Extensions
%\bibitem{distr} B. Mirzasoleiman, A. Karbasi, R. Sarkar, A. Krause, Distributed Submodular Maximization
\bibitem{recent}  T. Hess, S. Sabato, The monotone submodular secretary problem under a cardinality constraint with limited resources
\bibitem{norouzi} Beyond 1/2-Approximation for Submodular Maximization on Massive Data Streams
\bibitem{linear} B. Mirzasoleiman, A. Badanidiyuru, A Karbasi, J. Vondrak, A. Krause, Lazier Than Lazy Greedy
%\bibitem{swm} M. Kapralov, I. Post, J. Vondrak, Online Submodular Maximization: Beating 1/2 Made Simple
\bibitem{vahab} N. Korula, V. Mirrokni, M. Zadimoghaddam, Online Submodular Welfare Maximization Greedy Beats 1/2 in random order



@article{buchbinder2018online,
  title={Online Submodular Maximization: Beating 1/2 Made Simple},
  author={Buchbinder, Niv and Feldman, Moran and Garg, Mohit},
  journal={arXiv preprint arXiv:1807.05529},
  year={2018}
}


==> conclusion.tex <==
In this paper, we defined a relaxation of the submodular secretary problem with cardinality constraint. We allow the algorithm
to select more than $k$ elements, and the algorithm should output a subset of size $k$ among selected items.
We designed an algorithm with asymptotic
competitive ratio $R$ for any $R<1-1/e$. The total number of selections is only $O(k)$ elements. 
It is open  whether we can generalize this result to more general constraints such as matroid constraints.


==> impossible.tex <==
%\section{Impossibility Result}

In this section we provide an upper bound showing the following:

\hardness*

%\begin{theorem}
%There is no algorithm achieving asymptotic competitive ratio $7/8+\epsilon$ for submodular secretary problem using $o(n)$ selections. 
%\end{theorem}

%\mcomment{In the following proof we will consider a submodular $k+1$-secretary} problem. 
In the following proof, for simplicity of notation, we prove the desired bound for submodular $(k+1)$-secretary problem. %Since $k+1=O(k)$, the upper bound derived will imply the stated bound for the  submodular $k$-secretary problem. 
For any given $n, k$, we construct a set of instances of the  \nameOfProblemSLplus~such that any online algorithm that uses a shortlist of size $\eta(k+1)$ will have competitive ratio of at most $\frac{7}{8} + \frac{\eta(k+1)}{2n}$ on a randomly selected instance from this set. 

First, we define a monotone submodular function $f$ as follows. 
%For $n>0$, we define a  monotone submodular function $f$. 
The ground set consists of $\frac{n}{2k}+n-1$ items. There are two types of items, $C$ and  $D$, with $L:=n/2k$ items of type $C$ and
$n-1$ items of type $D$. We define $f(\phi):=0$, $f(\{c\}):=k$ for $c\in C$, and $f(\{d\}):=1$ for all $d\in D$. 
%There are infinitely many elements of $C$ and $D$. 
%\scomment{Don't you just need $L$ items of type $C$ and $n-1$ items of type $D$?}
%There are
Also there is a collection of $L$ {\it disjoint} sets $T_{\ell}=\{c^{\ell}, d_1^{\ell},\cdots, d^{\ell}_{k}\}$, $\ell=1,2, \ldots L$, such that $c^{\ell}\in C$ and $d_j^{\ell}\in D$. We define $f(T_{\ell}):=2k$ for all $\ell=1,\ldots, L$.
%\scomment{infinite number of such sets? or will $L$ suffice?} 
%\mcomment{in the definition of function it should be infinite but in the input we use $n/2k$ of them}
%\scomment{After going through the proof, I don't see why you need infinite number, it seems just $L=n/2k$ will suffice. Where are you using that there are infinte number of $T^\ell$?}
%\mcomment{
%The reason is that you should give one functions $f$ that works for all $n$. Otherwise one may claim that for any given function $f$ there is large enough $N_f$ so that we can go beyond 7/8, for $n>N_f$. 
%}
Now, let
$$g(t):=k+\frac{k}{2}+\cdots+ \frac{k}{2^{i-1}} + \frac{(t-ik)}{2^i},$$
where $i=\floor{t/k}$. It is easy to see that $g$ is a monotone submodular function. 

Now, define $f$ on the remaining subsets of the ground set as follows. For all $S$ with $|S|\ge 1$, 
\begin{itemize}
\item $|S\cap C| \ge 2 \implies f(S):=2k+1$
\item $|S\cap C|=0 \implies f(S):=1+g(|S|-1)$
\item $|S\cap C|=1$ $\implies S\cap C=\{c^\ell\}$ for some $\ell\in [L]$   $\implies$
%$$f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+\frac{k'}{2} (g(|S|-1)-g(|S|-2))\},$$ 
%$$f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+\frac{k'}{2^{i+1}}\},$$ 
$$f(S):= \min\{2k+1, k+\frac{1}{2} g(|S|-1)+\frac{k'}{2^{i+1}}\},$$ 
%\mcomment{so can we remove min above? }\scomment{yes, actually, you don't use $f(S)\le 2k+1$ anywhere, do you?} 
where $k'=|S\cap\{d^{\ell}_1,\cdots, d_k^{\ell}\} |$, $i=\lfloor(|S|-1)/k\rfloor$.
\end{itemize}

%\scomment{$i$ was not defined in above, please check if I defined it correctly.}
%\mcomment{yes}
%\scomment{isn't the first case in the below gone now?}
%\mcomment{no why?} \scomment{because all items in $C$ are $c^\ell$ for some $\ell$}
%\mcomment{yes correct}
%\scomment{removed below
%\begin{itemize}
%\item ..
%\begin{itemize}
%\item $S\cap C\notin\{c^{\ell}\}_{\ell=1, \ldots, L} \implies f(S):=k+\frac{1}{2} g(|S|-1)$
%\item $S\cap C= \{c_1^{\ell}\}$ for some $\ell$  $\implies f(S):=\min\{2k+1, k+\frac{1}{2} g(|S|-1)+k'/2^{i+1}\}$, where $k'=|S\cap\{d^{\ell}_1,\cdots, d_k^{\ell}\} |$.
%\end{itemize}
%\end{itemize}
%}
%Observe that for any subset $S$, $f(S)\le 2k+1$. 
Observe that since $g(k)=k$, for any subset $S$ of size at most $k+1$, we have $f(S)\le k+\frac{k}{2} + \frac{k}{2} = 2k$.

\begin{lemma}
$f$ is a monotone submodular function.
\end{lemma}
\begin{proof}
We have to show that for any item $x$ and subsets $S\subseteq T$, $\Delta_f(x|S) \ge \Delta_f(x|T)$.
We consider the following cases:
\begin{itemize}
\item if $|T\cap C| \ge 2 \implies \Delta_f(x|T)=0$, so it is trivial.
\item if $|T\cap C| =0 \implies |S\cap C|=0 \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.
\item if $|T\cap C|=1 \implies |S\cap C|\le 1$
\begin{itemize}
\item if $|S\cap C|=1 $ then $S\cap C = T\cap C = \{c^{\ell}\}$ for some $\ell$:
\begin{itemize}
\item $x\in \{d_1^{\ell},\cdots, d_k^{\ell}\} \implies \Delta_f(x|S)=1/2^{i+1}+1/2^{i+1}$ for $i=\lfloor (|S|-1)/k\rfloor$, and $\Delta_f(x|T)=1/2^j+1/2^j$ for some $j=\lfloor (|T|-1)/k\rfloor$ and $j\ge i+1$.
\item $x\notin \{d_1^{\ell},\cdots, d_k^{\ell}\} \implies \Delta_f(x|S)=1/2^{i+1}$ for $i=\lfloor (|S|-1)/k\rfloor$ and $\Delta_f(x|T)=1/2^j$ for some $j\ge i+1$.
\end{itemize} 
%\item $S\cap C = T\cap C \notin \{c_1^{\ell}\}_{\ell} \implies \Delta_f(x|S) \ge \Delta_f(x|T)$ because of submodularity of $g$.

\item if $|S\cap C|=0 \implies \Delta_f(x|T) \le 1/2^{j+1}+1/2^{j+1}$ for $j=\lfloor (|T|-1)/k\rfloor$ and $\Delta_f(x|S)= 1/2^i$ for some $i\le j$. 
\end{itemize}
Thus $\Delta_f(x|S) \ge \Delta_f(x|T)$.
\end{itemize} 
Monotonicity follows trivially from the definition of $f$.
\end{proof}

\toRemove{
Also for any subset of $S$ with at least two elements of $C$, $f(S)=2k$. 
For subset $S$ with no element in $C$, if $i=\floor*{\frac{|S|}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+k/2+ \dots +(|S|-ik)/2^{i}.
\]
For subset $S$ with exactly one element $c\in C$ such that $c\neq c_1$, if if $i=\floor*{\frac{|S|-1}{k}}$, 
$f(S)$ is defined as 
\[
f(S)= k+ k/2+ \dots +(|S|-1-ik)/2^{i+1}.
\]
Thus if $|S|=k+1$ and it contains exactly one element of $c\in C$ such that $c\neq c_1$ then $f(S)=k+k/2$.
Now suppose $S$  contains $c'$. 
For $S=T$, $f(S)=2k$.  Suppose $S$ contains $k'<k$ elements of $\{b_1, \dots, b_k\}$  and $\ell$ other elements of $D$. 
Let's $t=k'+\ell$, and $i=\floor*{\frac{t}{k}}$, then
\[
f(S)= \min\{2k, k'/2+(k+ k/2+ \dots +(t-ik)/2^{i+1})\}
\]
}
%\scomment{this proof is very vague, especially the claim any algorithm will select $k/2$ of $D$? Phrases like algorithm is not "aware" of something cannot be stated as a fact. You need to prove that the algorithm will not be able to distinguish between the two scenarios. We need to discuss.}



%Let $ {\cal T}^L$ be a collection of (any) $L=n/2k$ sets from $T^\ell, \ell=1,2, \ldots$. W.l.o.g., let's assume ${\cal T}^\ell = \{T_1, \ldots, T_L\}$.   

Now, denote $D^{\ell} := T^\ell \cap D = \{d_1^{\ell},\cdots, d_k^{\ell}\}$ for $\ell=1,2, \ldots, L$. Also, let 
$D'=D\setminus (\bigcup_{\ell=1}^L D^{\ell})$. % where $L:=n/2k$. 
%\scomment{Do you need $T^\ell, \ell =1,\ldots, L$ to be disjoint?} \mcomment{yes}
% $B'=B\setminus (\bigcup_{\ell }^{L} B^{\ell})$ for $L:=n/2k$.
Now define $L$ input instances $\{I_{\ell}\}_{\ell =1,\ldots, L}$, each of size $n$, as follows. For
any arbitrary subset $\tilde{D}\subseteq D'$ of size $n-Lk-1$, 
%\scomment{Which subset $\tilde{B}$? any arbitrary subset?} \mcomment{arbitrary}
define $I_{\ell}=\bigcup_{i=1,\ldots, L}  D^{i} \cup \tilde{D} \cup \{c^{\ell}\}$, for  $\ell=1,\ldots, L$.
%and $I_2=B^1 \cup B^2 \cup \tilde{B} \cup \{a_1^2\}$ (the difference is $a_1^1$ and $a_1^2$).
%Now suppose the input consists of the following:  $T^{\ell}=\{a_1^{\ell}, b_1^{\ell}, \cdots b_k^{\ell} \}$, no other element of $C$ and the remaining elements are from $B':=B\setminus \{b_1^{\ell}, \cdots, b_k^{\ell}\}$. 
Thus, for instance $I_{\ell}$, the the optimal $k+1$ subset is $T^\ell$ with value $f(T^{\ell})=2k$. 
%\scomment{earlier we stated $T^\ell$ is optimal, but we have never proven that none of the $k+1$ subset can take value $2k+1$. We actually do not need to show $T^\ell$ is optimal.}
%\scomment{$T^\ell$ is of size $k+1$, optimal should be of size $k$. If making $T_\ell$ to be of size $k$ makes it messy, you can initially state that you will consider submodular $k+1$ secretary problem.}


Now consider any algorithm for the submodular \nameSecSL\ and cardinality constraint $k+1$. We denote by $Alg$ the set of $\eta(k+1)$ items selected by the algorithm as part of the shortlist. % (all elements in the shortlist of size $\eta(k)$).
%\scomment{We have  used $C$ to denote shortlist in the algorithm. May be you can use a different symbol instead of type $A$ and $B$. }
Let $\bar I$ denote an instance chosen uniformly at random from $I_\ell, \ell=1,\ldots, L$.  
%We choose one of $I_{\ell}$ randomly. \scomment{randomly or arbitrarily?} 
Let $\pi$ denote a random ordering of $n$ items in $\bar I$. 
%We give a random order of $I_{\ell}$, say $\pi$ to the algorithm as input,
%(note that in the secretary problem the elements of input can be selected adversarially but the order should be random).
We denote by random variable $(\bar{I},\pi)$ the randomly ordered input instance to the algorithm. Also we denote by $\bar{T}, \bar{D}$ and $\bar c$, the corresponding $T^{\ell}$, $D^{\ell}$ and $c^\ell$.

Now we claim 

%Note that algorithm is not aware of $\ell$.
%Consider an algorithm $Alg$.
%Suppose $a_1^{\ell}$ is the $t$-th elements in the input, and
%elements of input are ordered as $I=(I_1,\cdots, I_n)$.
%Suppose $Alg$ is the set of elements selected by an algorithm.
%Denote by $\bar{B}=\{b_1,\cdots, b_k\}$.

\begin{lemma}
$\mathbb{E}_{(\bar{I},\pi)}[|Alg\cap \bar{D}|] \le k/2+\eta(k+1)/L$.
\end{lemma}
\begin{proof}
Suppose $(e_1,\cdots, e_n)$ indicates the ordered input according to random ordering $\pi$ on $\bar{I}$. %for some $0<\ell<L$.
Now let $t$ be the random variable indicating the index of $c^{\ell}$ in $(e_1,\cdots, e_n)$, i.e., $e_t=c^{\ell}$. 
%Define $R:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}|]$.
Then, due to random ordering, and random choice of $\bar I$ from $I_1, \ldots, I_\ell$, we have
$$\mathbb{E}_{(\bar I, \pi)}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap D^1|]= \cdots = \mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap D^{L}|]\ .$$
Also, since $D^\ell, \ell=1,\ldots, L$ are disjoint,
$$\sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap D^{\ell}|] \le \eta(k+1)\ .$$
Since $\bar D=D^\ell$ with probability $1/L$,  we have
$$H:=\mathbb{E}[|Alg\cap\{e_1,\cdots, e_{t-1}\}\cap \bar{D}|]=  \frac{1}{L} \sum_{\ell=1}^L \mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\}\cap D^{\ell}|] \le \frac{1}{L} \eta(k+1)\ . $$ 
%\rightarrow 0$ as $n/\eta(k) \rightarrow \infty$.
Now define
$G:=\mathbb{E}[|Alg\cap\{e_t,\cdots, e_{n}\}\cap \bar{D}|]$.
We have
$$G\le \mathbb{E} [|\bar{D}\cap\{e_t,\cdots, e_n\}|]  \le k/2\ .$$
%Also define $H:=\mathbb{E}[|Alg\cap\{e_1,\cdots,e_{t-1}\cap \bar{B}\}|]$.
%Also, $H\le k-G$.
Thus $$\mathbb{E}[|Alg\cap \bar{D}|] \le G+H\le k/2+\eta(k+1)/L\ .$$
%\rightarrow G$$
%\le k/2$$
%G+(k-G)/2 \le k/2+G/2\le k/2+k/4=3/4k$$.
\end{proof}
Now on input $\bar{I}$, if the algorithm doesn't select $\bar c$ as part of shortlist $Alg$, then by definition of $f$ for sets that do not contain any item of type $C$, we have 
$$f(A^*):=\max_{S \subseteq Alg:|S|\le k+1} f(S) \le 1+ g(k) = k+ \frac{k}{2}$$ 

Otherwise, if algorithm selects $\bar c$ then by definition of $f$ 
$$f(A^*):=\max_{S \subseteq Alg:|S|\le k+1} f(S) \le \max_{S \subseteq Alg \backslash (\bar D \cup \{\bar c\}):|S|\le k-|Alg \cap \bar D|} f(S \cup \bar D \cup \{\bar c\}) 
= k+ \frac{k}{2} +\frac{1}{2} |Alg\cap \bar{D}|$$ 
therefore $$\mathbb{E}[f(A^*)] \le k+\frac k 2+ \frac k 4+ \frac{\eta(k+1)}{2L} = \frac{7k}{4} + \frac{k\eta(k+1)}{n} \ .$$

%Hence $\mathbb{E}[f(Alg)]  \rightarrow k+k/2+k/4$ as $n\rightarrow \infty$, since $\eta(k)=o(n)$.
Since the optimal is equal to $\Ex[f(\bar T)]=2k$, the competitive ratio is upper bounded by
$$ 
%\left(\frac{7k}{4} + \frac{k\eta(k)}{n}\right)\left/\right. 2k = 
\frac{7}{8} + \frac{\eta(k+1)}{2n}$$

This proves competitive ratio upper bound of $\frac{7}{8} + o(1)$ when $\eta(k+1)=o(n)$, to complete the proof of Theorem \ref{hardness}.
%\scomment{I think we need to change the upper bound in theorem statement to $7/8 + o(1)$}
%Before arriving $a_1^{\ell}$ algorithm can not distinguish between elements of $B'=\{b_1^{\ell},\dots, b_k^{\ell}\}$
%and the rest of $D$ thus the expected number of elements in $B'$ selected by algorithm before observing $a_1$ goes to $0$ as $n/k\rightarrow \infty$.

%Therefore an online algorithm would select $k/2$ elements of set $B'$ in expectation and also it selects $a_1^{\ell}$ (and $k/2$ other elements from $B\setminus B'$).  Therefore, its $f$ value is $k+k/2+k/4$.
%Hence the competitive ratio is at most $7/8$.


==> introduction.tex <==
%\section{Introduction}



In the classic \textit{secretary problem}, 
$n$ items appear in random order.  We know $n$, but don't know the value of an item until it appears.   
Once an item arrives we have to irrevocably and immediately decide whether or not to select it. Only one item is allowed to be selected, and the objective is to  select the most valuable item, or perhaps to 
%\ccomment{Is this really equivalent, or just related}
%\mcomment{not equivalent but related. }
maximize the expected value of the selected item  
%The origin of the secretary problem is hard to track
~\cite{Dynkin:SovMath:1963,ferguson1989solved, 10.2307/2985407}. 
It is well known that the optimal policy is to observe the first $n/e$ items without making any selection and then select the first item whose value is larger than the value of the best item in the first $n/e$ items~\cite{Dynkin:SovMath:1963}. This algorithm, given by ~\citet{Dynkin:SovMath:1963},
is asymptotically optimal, and hires the best secretary with probability at least $1/e$. Hence it
is also $1/e$-competitive for the expected value of the chosen item, and
%\ccomment{Is this true?}
%\mcomment{Yes, but the original paper shows the probability not the expectation Dynkin provided an asympotically optimal algorithm for this problem, which hires the best secretary with probability at least 1/e}
it can be shown that no algorithm can beat $1/e$-competitive ratio in expectation.
%

Many variants and generalizations of the secretary problem have been studied in the literature, see e.g., \cite{Ajtai:2001,WILSON1991325,vanderbei1980optimal, wilson1991optimal, kleinberg, Babaioff:2008}.  
%\ccomment{We should have more variants hear} The secretary problem has been generalized.  
\cite{kleinberg, Babaioff:2008} introduced a 
{multiple choice secretary problem}, where the goal is to select $k$ items in a randomly ordered input so as to maximize  the {\it sum} of their values; and  \citet{kleinberg} gave an algorithm with an asymptotic competitive ratio of $1-O(1/\sqrt{k})$. Thus as $k\to \infty$, the competitive ratio approaches  1. Recent literature studied several generalizations of this setting to multidimensional knapsacks \cite{moser1997algorithm}, and proposed algorithms for which the expected online solution approaches the best offline solution as the knapsack sizes becomes large~(e.g., \cite{FHKMS10, devanur-hayes, AgrawalWY14}). 


In another variant of multiple-choice secretary problem, \citet{Bateni} and ~\citet{Gupta:2010} introduce 
the \textit{\nameOfProblem}. In this secretary problem, the algorithm again selects $k$ items, but 
the value of the selected items is given by a monotone submodular function 
%It is an online variant of monotone submodular maximization subject to cardinality constraints. 
%The objective function is designed by an adversary, but the order of the items is uniformly at random.
$f$. The algorithm has a value oracle access to the function, i.e., for any given set $T$, an algorithm can query an oracle to find its value $f(T)$~\cite{oracle}.
The algorithm can select at most $k$ items $a_1 \cdots, a_k$, from a randomly ordered sequence of $n$ items. The goal is to maximize $f(\{a_1,\cdots, a_k\})$.
%Now imagine we are allowed to select several items instead of one item. Would that let us to improve $1/e$?
%Assuming a value oracle access to the submodular function; i.e., for a given set $T$, an algorithm can query an oracle to find its value $f(T)$~\cite{oracle}.
Currently, the best result for this setting is due to ~\citet{kesselheim}, who achieve a $1/e$-competitive ratio in exponential time, or $\frac{1}{e}(1-\frac{1}{e})$ in polynomial time. In this case, the offline problem is NP-hard and hard-to approximate beyond the factor of $1-1/e$ achieved by the greedy algorithm \cite{nemhauser1978best}. 
%\scomment{need a reference for lower bound of $1-1/e$ for offline monotone submodular maximization}
However, it is unclear if a competitive ratio of $1-1/e$ can be achieved by an online algorithm for the {\nameOfProblem} even when $k$ is large. 

\paragraph{Our model: \nameSecSL.}
In this paper, we consider a relaxation of the secretary problem 
%.  What if  the online algorithm for secretary problem 
where the algorithm is allowed to  select a {\it shortlist} of items that is larger than the number of items that ultimately need to be selected. That is, in a multiple-choice secretary problem with cardinality constraint $k$, the algorithm is allowed to choose more than $k$ items as part of a shortlist. Then, after seeing the entire input, the algorithm can choose a subset of size $k$ from the bigger set of items in the shortlist. 
%when seeing items online, and ultimately maximizes a function of $k$ elements, 
%we are allowed to choose more than $k$ elements, and then after seeing the entire input, choose a  a subset of size $k$ from our bigger set.  

This new model is motivated by some practical applications of secretary problems, such as hiring (or assignment problems),  where in some cases it may be possible to tentatively accept a larger number of candidates (or requests), while deferring the choice of the final $k$-selections to after all the candidates have been seen. Since there may be a penalty for declining candidates who were part of the shortlist, one would prefer that the shortlist is not much larger than $k$.

Another important motivation is theoretical: we wish to understand to what extent this relaxation of the secretary problem can improve the achievable competitive ratio. This question is in the spirit of several other methods of analysis that allow an online algorithm to have additional power, such as {\em resource augmentation} \cite{KalyanasundaramP00,PhillipsSTW97}.

The potential of this relaxation is illustrated by the basic secretary problem, where the aim is to select the item of maximum value among randomly ordered inputs. There, it is not difficult to show that if an algorithm  picks every item that is better than the items seen so far, the true maximum will be found, while the expected number of items picked under randomly ordered inputs will be $\log(n)$. Further, we show that this approach can be easily modified to get the maximum with $1-\epsilon$ probability while picking at most  $O(\ln(1/\epsilon))$ items for any constant $\epsilon>0$. Thus, with just a constant size shortlist, we can break the $1/e$ barrier for the secretary problem and achieve a competitive ratio that is arbitrarily close to $1$.

%For the secretary problem, we can imagine choosing not one secretary, but several, and then taking the best one at the end.  
Motivated by this observation, we ask if a similar improvement can be achieved by relaxing the \nameOfProblem~to allow a shortlist. That is, instead of choosing $k$ items, the algorithm is allowed to chose  $\eta(k)$ items as part of a shortlist, for some function $\eta$;
and at the end of all inputs, the algorithm chooses $k$ items from the $\eta(k)$ selected items. Then, what is the relationship between $\eta(\cdot)$ and the competitive ratio for this problem? Can we achieve a solution close to the best offline solution when $\eta(k)$ is not much bigger than $k$, for example  when 
 $\eta(k)=O(k)$?  

%We answer this question affirmatively in this paper, and provide an algorithm 
%What is the relationship between $\eta$ and the competitive ratio. 
%In other words, we have a {\em shortlist} of size $\eta(k)$, where $\eta(k)$ is independent of $n$, and the output is subset of this shortlist.
%We wish to understand how much this relaxation can improve the competitive ratio.   In other words, what is the relationship between $\eta$ and the competitive ratio.
 
%For exmaple, when the  it is possible to approach the optimal offline solution by some function $\eta$ as $k\to \infty$.  Can we obtain a similar results for the \nameOfProblemSL.


%\ccomment{Is there a practical-ish motivation for this model?}
%A motivation for this model is that for the $k$-secretary problem instead of restricting ourselves to make irrevocable decisions for each item, we may add items to a shortlist and defer the final decision to the end (choosing $k$ elements from shortlist). We want the size of shortlist to be as small as possible.

In this paper, we answer this question affirmatively by giving a polynomial time algorithm that achieves $1-1/e-\epsilon-O(k^{-1})$ competitive ratio for the \nameOfProblem~using a shortlist of size $\eta(k)=O(k)$. This is surprising since $1-1/e$ is the best achievable approximation (in polynomial time) for the offline problem. Further, for some special cases of submodular functions, we demonstrate that an $O(1)$ shortlist allows us to achieve a $1-\epsilon$ competitive ratio. These results demonstrate the power of (small) shortlists for closing the gap between online and offline (polynomial time) algorithms. 
%size we give a new algorithm and show several positive (and one negative) results that capture the power of these shortlists and  show that they are (surprisingly) powerful. 

We also discuss connections of {\nameSecSL} to the related streaming settings. While a streaming algorithm does not qualify as an online algorithm (even when a shortlist is allowed), we show that our algorithm can in fact be implemented in a streaming setting to use $\eta(k)=O(k)$ memory buffer; and our results significantly  improve  the available results for the \streamingProblem.
Furthermore since the upperbound given in ~\cite{mcgregor2017better} holds for random order streams, our result is asymptotically tight in this setting.

\subsection{Problem Definition}
%In the well-studied submodular $k$-secretary problem, applicants from a set ${\cal U} = \{a_1, a_2, \ldots, a_n\}$  (pool of applicants) arrive in a uniformly random order over $n$ sequential rounds. In each round, an online algorithm irrevocably decides whether to select an applicant or not. The algorithm can select at most $k$ applicant. The goal is to maximize the value of the selected $k$ applicants, as given by a submodular function $f$. 

%More formally, let $S, |S|\le k$ denote the subset of candidates selected by the algorithm, then the expected utility of the algorithm is given by $\ALG:=\Ex[f(S)]$, where $f$ is a monotone submodular function, and the expectation taken both over random order and possible randomness in the algorithm's selection of subset $A$ given an order. The competitive ratio of the online algorithm is then defined as $\frac{\ALG}{\OPT}$, where $\OPT$ is the optimal offline utility defined as 
%$$\OPT=f(S^*), \text{ where, } S^*=\arg \max_{S \subseteq [n], |S|\le k} f(S).$$

%\scomment{edited by me on 8/21}
We now give a more formal definition.
Items from a set ${\cal U} = \{a_1, a_2, \ldots, a_n\}$  (pool of items) arrive in a uniformly random order over $n$ sequential rounds. The set ${\cal U}$ is apriori fixed but unknown to the algorithm, and the total number of items $n$ is known to the algorithm. In each round, the algorithm irrevocably decides whether to add the arriving item to a {\it shortlist} $A$ or not. %The goal is to return,  at the end of $n$ rounds, a shortlist $A$ of size at most $\eta(k) \ge k$ to maximize the  `value' of best $k$ subset of this shortlist. More formally, 
%We are given a monotone submodular function $f:2^{\cal U} \rightarrow \mathbb{R}$, in a value oracle model. %Let the set $A \subseteq {\cal U}, |A|\le \eta(k)$ denote the shortlist of items selected by the online algorithm,  then 
The algorithm's value at the end of $n$ rounds is given by 
$$\ALG = \Ex[\max_{S\subseteq A, |S|\le k} f(S)]$$ 
where $f(\cdot)$ is a monotone submodular function. The algorithm has value oracle access to this function.

The optimal offline utility is given by
$$\OPT:=f(S^*), \text{ where } S^*=\arg \max_{S \subseteq [n], |S|\le k} f(S).$$ 
We say that an algorithm for this problem achieves a competitive ratio  $c$ using shortlist of size $\eta(k)$, if at the end of $n$ rounds, $|A|\le \eta(k)$ and $\frac{\ALG}{\OPT}\ge c$.

Given the shortlist $A$, since the problem of computing the solution $\arg \max_{S\subseteq A, |S|\le k} f(S)$ can itself be computationally intensive, our algorithm will also track and output a subset $A^* \subseteq A, |A^*| \le k$. We will lower bound  the competitive ratio by bounding $\frac{f(A^*)}{f(S^*)}$.

The above problem definition has connections to some existing problems studied in the literature. The well-studied online \nameOfProblem~described earlier is obtained from the above definition by setting $\eta(k)=k$, i.e., it is same as the case when no extra items can be selected as part of a shortlist. 
%\scomment{Did a pass on the para below on 8/30 after our discussion regarding streaming problem}
Another related problem is {\it  \streamingProblem}~studied in~\cite{norouzi}. In this problem, items from a set $\cal U$ arrive online in random order and the algorithm aims to select a subset $S \subseteq {\cal U}, |S|\le k$ in order to maximize $f(S)$. The streaming algorithm is allowed to maintain a {\it buffer} of size $\eta(k)\ge k$. 
However, this streaming problem is distinct from the \nameOfProblemSL\ in several important ways. On one hand, since an item previously selected in the memory buffer can be discarded and replaced by a new items, a memory buffer of size $\eta(k)$ does not imply a shortlist of size at most $\eta(k)$. On the other hand, in the secretary setting, we are allowed to memorize/store more than $\eta(k)$ items without adding them to the shortlist. Thus an algorithm for \nameOfProblem with shortlist of size $\eta(k)$ may potentially use a buffer of size larger than $\eta(k)$. 
Our algorithms, as described in the paper, do use a large buffer, but we will show
%\ccomment{Where do we show that the streaming actually works}
that the algorithm presented in this paper can in fact be implemented to use only $\eta(k)=O(k)$ buffer, thus obtaining matching results for the streaming problem. 
%imply the same competitive ratio for random order streaming problem with buffer of size $\eta(k)$, but not vice-versa. We will discuss the corollary of our algorithm design and analysis for the  submodular random order streaming problem. 
%Because shortlists can be used as a buffer for memory but not vice versa. ( we are allowed to delete from memory and reduce the size but we can not remove from a shortlist)







%In the new `submodular $k$-secretary with shortlist' problem considered in this paper, we allow the online algorithm to select a shortlist of more than $k$ candidates, and pick the final subset of $k$ candidates from this shortlist at the end. Specifically,  we allow the online algorithm to select a subset $A$ of size $|A|\le \eta(k)$, where $\eta(k)\ge k$. The competitive ratio of the online algorithm is then defined with respect to the best $k$-subset of $A$. That is, competitive ratio is given by $ \frac{\ALG_{\eta}}{\OPT}$, where $\OPT$ as defined before, and 
%$$\ALG_\eta = \Ex[\max_{S\subseteq A, |S|\le k} f(S)],$$ 
%with $A$ being the subset of items selected by the online algorithm, of size at most $\eta(k)$. 

\subsection{Our Results}
Our main result is an online algorithm  for \nameOfProblemSL\ that, for any constant $\epsilon>0$, achieves a competitive ratio of $1-\frac{1}{e} - \epsilon-O(\frac{1}{k})$ with $\eta(k) = O(k)$. 
Note that for \nameOfProblem\ there is an upper bound of $1-1/e$ on the achievable aproximation factor, even in the offline setting, and this upper bound applies to our problem for arbitrary size $\eta(\cdot)$ of shortlists. On the other hand for online monotone \nameOfProblem, i.e., when $\eta(k)=k$, the best competitive ratio achieved in the literature is $1/e-O(k^{-1/2})$~\cite{kesselheim} 
%\scomment{is there an upper bound? } \mcomment{ No} 
Remarkably, with only an $O(k)$ size shortlist, our online algorithm is able to achieve a competitive ratio that is arbitrarily close to the offline upper bound of $1-1/e$.

In the theorem statements below, big-Oh notation $O(\cdot)$ is used to represent asymptotic behavior with respect to $k$ and $n$. We assume the standard  value oracle model:  the only access to the submodular function is through a black box
returning $f(S)$ for a given set $S$, and  each such queary can be done in $O(1)$ time. 
%\ccomment{Define value oracle model and state thm.1 appropriately}
\begin{theorem} \label{opttheorem}
For any constant $\epsilon>0$, there exists an online algorithm (Algorithm \ref{alg:main}) for the \nameOfProblemMatroidSL\ that achieves a competitive ratio of $1-\frac{1}{e} -\epsilon -O(\frac{1}{k})$, with shortlist of size $\eta_\epsilon(k)=O(k)$. Here,  $\eta_\epsilon(k)=O(2^{poly(1/\epsilon)}k)$.  
%$$\eta_\epsilon(k) =c k\log(1/\epsilon) {\frac{1}{\epsilon^3} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^2} \log(1/\epsilon)}} =O(2^{poly(1/\epsilon)}) \ ,$$
%for some absolute constant $c$.
% for submodular secretary problem with cardinality constraints, such that it selects $O(k)$ elements. %, where $C(a)$ is a constant depending only on $a$.
  The running time of this online algorithm is $O(n)$.
\end{theorem}

Similar to~\cite{us}, an interesting aspect of our algorithm is that it is highly parallel. Even though the decision for each arriving item may take time that is exponential in $1/\epsilon$ (roughly  $\eta_\epsilon(k)/k$), it can be readily parallelized among multiple (as many as $\eta_\epsilon(k)/k$) processors. 
%The  operations required to make a decision for each item can be divided between available processors. (the running time will be divided by $\min(c,p)$ where $c=k\log(1/\delta) {\frac{1}{\delta^3} \log(1/\delta)  \choose {\frac{1}{\delta^2} \log(1/\delta)}}$ is the hidden constant in $O(k)$ and $p$ the number of processors )


%More precisely, we design a $1-1/e-\epsilon-O(k^{-1})$ competitive algorithm that selects $O(k\log(1/\delta) {\frac{1}{\delta^3} \log(1/\delta)  \choose {\frac{1}{\delta^2} \log(1/\delta)}})$ elements, i.e., the dependency on $k$ is linear and on $\delta$ is exponential.



%\scomment{Add a formal corollary of Theorem 1 for random-order streaming problem here. Also, will be good to add a few lines in problem definition section describing how our problem relates to random order streaming.} \mcomment{done done}


%As discussed earlier, by definition, a corollary of our results is an algorithm for the submodular random order streaming problem with the same competitive ratio.
Further, we show an implementation of Algorithm 2 that uses a memory buffer of size at most $\eta_\epsilon(k)$ to get the following result for the problem of {\it \streamingProblem} described in the previous section. 
%\ccomment{Make terminology for evaluations consistent with previous work}
\begin{restatable}{theorem}{thmStreaming}
\label{thm:streaming}
For any constant $\epsilon\in (0,1)$, there exists an algorithm for the \streamingProblem  that achieves $1-\frac{1}{e} -\epsilon -O(\frac{1}{k})$ approximation to $\OPT$ while using a memory buffer of size at most $\eta_\epsilon(k)=O(k)$. Also, the number of objective  function evaluations for each item, amortized over $n$ items, is $O(1+\frac{k^2}{n})$.
%Also, decision for each arriving item requires $O(1)$ evaluations of the objective function.
%Also in amortized time, it processes each arriving item with $O(1+\frac{k^2}{n})$ evaluations of the objective function.
%Also the amortized time to processes each arriving item requires $O(1+\frac{O(k^2)}{n})$ evaluations of the objective function.
% The running time of this online algorithm is $O(n)$.
\end{restatable}
%The above result significantly improves over the state-of-the-art results in random order streaming model \cite{norouzi}, which are an approximation ratio of $\frac 1 2+8\times 10^{-14}$ using a memory of size $O(k\log k)$. 
%uses $O(k)$ memory and achieves asymptotic $R<1-1/e$ approximation.

%\scomment{I don't understand the upper bound stated below - by arbitrary $\eta$, couldn't we get at best the the offline problem. I can just select everything into shortlist. So, is the below giving an upper bound for the offline problem?  } \mcomment{using $o(n)$ selections. No it is for online problem}

%As a result, we show that in our model $\eta(k)=\gamma.k$, where $\gamma$ is a constant. It is optimal up to a constant factor.
%The constant factor $\gamma$ is growing as the competitive ratio gets closer to $1-1/e$. 
%Because of the known upper bound for offline submodular maximization with cardinality constraint.
%It is obvious that we can not get better than $1-1/e$ competitive algorithm if we only consider  polynomial time algorithms. 

%It is natural to ask whether these $k$-lists are, in fact, too powerful.  Maybe they could actually allow us to always match the best offline algorithm.  We give a negative result in this direction and 
%show that even if we have unlimited computation power, for any function $\eta(k)=o(n)$, we can get no better than $7/8$-competitive algorithm using a shortlist of size $\eta(k)$. Note that with unlimited computational power, the offline problem can be solved exactly. This result demonstrates that 
%having a shortlist does not make the online problem too easy - 
%even with a shortlist (of size $o(n)$) there is an information theoretic gap between the online and offline problem. Note that the $1-1/e$ upperbound for streaming model~\cite{mcgregor2017better} 
%does not imply an upper bound for the shortlist model.

\toRemove{
%\mcomment{we should emphasize the upper bound is for any $k$, i.e., it holds asymptotically}
\begin{restatable}{theorem}{hardness}
%\begin{theorem} 
\label{hardness}
No online algorithm (even with unlimited computational power)   can achieve a competitive ratio better than $7/8+o(1)$ for the \nameOfProblemSL, while using a shortlist of size $\eta(k)=o(n)$.
%by selecting $\eta(k)$ elements for any function $\eta$ (independent of $n$).
\end{restatable}
%\end{theorem}

%\scomment{By independent of $n$, do you mean $\eta(k)$ does not grow with $n$, i.e., $\eta(k)=O(1)$ if $O(\cdot)$ denotes asymptotic with respect to $n$? This is not same as $o(n)$, e.g.. $\eta(k)=\sqrt{n}$ would also be $\eta(k)=o(n)$.} \scomment{We need to discuss this issue}
 
 % It also improves~\cite{Badanidiyuru2014StreamingFly} on random order inputs.
%(Note that in our algorithm we keep extra items in the shortlist only for a limited time $O(n/k)$, and then we are able to release them.
%That is why the extra memory is $O(1)$ instead of $O(k)$).

%Another interesting aspect of our algorithm is that it is highly parallel. In order to decide whether or not to select an item in a slot $s_i$ in window $W$ which consists of $\{s_1, \dots, s_{\alpha \beta}\}$,
%the algorithm concurrently run several online maximum algorithms to find the maximum marginal value with respect to %different subsets.
% $S\cup \gamma(\tau)$, where $\tau$ is a subset of slots $\{s_1,\dots, s_{i-1}\}$ with $|\tau|<\alpha$.
%We select a new item if any of the maximum algorithms (for some $\tau$) select it, otherwise we do not select it. All the maximum algorithms for different subsets $\tau$ can be run in parallel. 

%Although the update time in our algorithm is $O(1)$, the constant can be very large. Consequently it may not be desirable for large streams. 
%We take two approaches to improve it. The first approach is parallel algorithms. The interesting fact about our algorithm is that it is highly parallel, i.e. the  operations required for each element can be divided between as many processor as it is available. 
%The running time will be divided by the number of processors. 

%In addition, we design a fast  thresholding algorithm that requires only one function evaluation per element.
%It achieves competitive ratio $1/2-O(1/\sqrt{k})$ by selecting $k\log^2k$ elements. The competitive ratio and the update time of this algorithm is still better than~\cite{kesselheim} and~\cite{Hess}. In ~\cite{kesselheim}  update time is $O(n^2)$. 
%In terms of memory, our thresholding algorithm uses less memory than~\cite{Badanidiyuru2014StreamingFly} but more than~\cite{Hess}.


%We also provide an upper bound showing that it is not possible to achieve any competitive ratio better than $7/8$ by selecting $O(g(k))$ elements, where $g$ is an arbitrary function, even if we have free computation.
%\scomment{Can you add a theorem statement for the results discussed below?} \mcomment{added}
Finally, for some special cases of monotone submodular functions, we can asymptotically approach the optimal solution.
%\ccomment{Don't mention this as a thm.}
%\begin{theorem}
%Suppose $F$ is a monotone submodular function and $F(a_1,\cdots, a_i+\alpha,\cdots, a_k)  \ge  F(a_1, \cdots, a_i, \cdots, a_k  )$, for any  $\alpha >0$ and $1\le i \le k$.
%Let $S$ be the elements selected by Kleinberg's algorithm~\cite{kleinberg}, then
%$E[F(S)]>(1-5/\sqrt{k})OPT$.
%%Let $T$ be the $k$ largest elements of $S$, and $OPT=f(T)$.
%The expected number of elements of $T$ selected by the algorithm is at least $(1 -5/\sqrt{k})k$.
%\end{theorem}
%\begin{enumerate}
%\item $F$ is a monotone submodular function, and $F(a_1,\cdots, a_i+\alpha,\cdots, a_k)  \ge  F(a_1, \cdots, a_i, \cdots, a_k  )$, for $\alpha >0$ and $1\le i \le k$.
%\end{enumerate}
%We show Kleinberg's algorithm asymptotically approaches optimal solution.
%We prove that the Kleinberg algorithm works under this assumption which means that the competitive ratio of the algorithm asymptotically approaches 1.
The first one is the family of functions we call $m$-submdular. 
A function $f$ is $m$-submodular if it is submodular and there exists a submodular function $F$ such that for all $S$:
%\begin{itemize}
%\item 
\[ 
f(S)= \max_{T\subseteq S, |T|\le m} F(T) \ .
\]
%\end{itemize}
\scomment{This needs to be rewritten, I don't have time right now, so removing: Example of $m$-submodular functions are   maximum node weighted bipartite matching and  maximum edge weighted bipartite matching defined on $G=(X\times Y)$ with $|Y|=m$.  (the assignments will be done at the end of algorithm after all the selections are made).}

%\scomment{
%What is $\epsilon, \delta$? I removed this and restated inline with our rest of the results.
%\begin{theorem}
%For any $m$-submodular function $F$ there is an Algorithm that selects a set $S$ with $|S|<m\ln (1/\epsilon)+\ln(1/\delta)+\sqrt{\ln^2{1/\delta}+2m\ln(1/\delta)\ln(1/\epsilon)}$ and $E[F(S)]=(1-\epsilon-\delta)OPT$.
%\end{theorem}
%}
%\begin{restatable}{theorem}{msub}
\begin{theorem}
\label{thm:msub}
If $f$ is an $m$-submodular function, there exists an online algorithm for the \nameOfProblemSL~that achieves a competitive ratio of $1-\epsilon$ with shortlist of size $\eta_{\epsilon,m}(k)=O(1)$. Here, 
$\eta_{\epsilon,m}(k) = (2m+3) \ln(2/\epsilon)$.
\end{theorem}
%\end{restatable}
A proof of Theorem~\ref{thm:msub} along with the relevant algorithm (Algorithm \ref{alg:SIII}) appears in the appendix.

Another special case  is  monotone submodular functions $f$ satisfying the following property:
$f(\{a_1,\cdots, a_i+\alpha,\cdots, a_k\})  \ge  f(\{a_1, \cdots, a_i, \cdots, a_k \})$, for any $\alpha >0$ and $1\le i \le k$.
We can show that the algorithm by \citet{kleinberg} asymptotically approaches optimal solution for such functions, but we omit the details.

}





%We call an algorithm $ALG$ c-competitive if for any objective function $F$ chosen by the adversary, the
%set of selected items $ALG$ satisfies $E [F(ALG)] \ge (c ? o(1)) · OPT$, where $OPT$ is a feasible
%(offline) solution that maximizes v and the o(1)-term is asymptotical with respect to the length of
%the sequence n. 










%What is the minimum size shortlist to get a  $c$-competitive algorithm?
%These are questions that we consider in this paper.



%The submodular secretary problem, introduced by Bateni2013SubmodularExtensions et al. and Gupta et al., is an
%online variant of monotone submodular maximization subject to cardinality constraints. In this
%problem, we are allowed to select up to k items from a set of n items.
%The value of a set is represented by a monotone, submodular function.
%The values of the submodular function are only known on subsets of the items that have already arrived.
%The objective function is designed by an adversary, but the order of the items is uniformly at random.




%It is well-known since 1963 [10]
%that the optimal policy is to interview the first t ? 1 applicants, then hire the next one whose quality exceeds that of
%the first t ? 1 applicants, where t is defined by ; as $n \to \infty$, the probability of hiring
%the best applicant approaches 1/e, as does the ratio t/n.
%Note that a solution to the secretary problem immediately
%yields an algorithm for a slightly different objective function optimizing the expected value of the chosen element.





%In secretary problem, we are given a random order input and we are going to select the maximum element.
%In the classic secretary problem, one is presented a sequence of items with different scores online in
%random order. Upon arrival of an item, one has to decide immediately and irrevocably whether to
%accept or to reject the current item.  The objective is to accept the best of these items. 




%Multiple Choice secretary problem:


%Submodular Secretary problem:



%Our extension


%Streaming model:





% Imagine that you
%manage a company, and you want to hire a secretary from a pool of n applicants. You are very keen on hiring only
%the best and brightest. Unfortunately, you cannot tell how good a secretary is until you interview him, and you must
%make an irrevocable decision whether or not to make an offer at the time of the interview. The problem is to design
%a strategy which maximizes the probability of hiring the most qualified secretary. It is well-known since 1963 [10]
%that the optimal policy is to interview the first t ? 1 applicants, then hire the next one whose quality exceeds that of
%the first t ? 1 applicants, where t is defined by ; as $n \to \infty$, the probability of hiring
%the best applicant approaches 1/e, as does the ratio t/n. Note that a solution to the secretary problem immediately
%yields an algorithm for a slightly different objective function optimizing the expected value of the chosen element.




%In this paper, we consider general monotone submodular functions.



%The submodular secretary problem, introduced by Bateni2013SubmodularExtensions et al. and Gupta et al., is an
%online variant of monotone submodular maximization subject to cardinality constraints. In this
%problem, we are allowed to select up to k items from a set of n items.
%The value of a set is represented by a monotone, submodular function.
%The values of the submodular function are only known on subsets of the items that have already arrived.
%The objective function is designed by an adversary, but the order of the items is uniformly at random.

%We call an algorithm c-competitive if for any objective function v chosen by the adversary, the
%set of selected items ALG satisfies $E [v(ALG)] \ge (c ? o(1)) · v(OPT)$, where $OPT$ is a feasible
%(offline) solution that maximizes v and the o(1)-term is asymptotical with respect to the length of
%the sequence n. 

\scomment{The susection "Our techniques" was describing analysis and algorithm design techniques that are not being used in the proof anymore, there is no time to revise it, so I am removing it. Most of this intuition appears in algorithm description and proof overview anyway.}
\toRemove{
\subsection{Our techniques}
First we design a simple algorithm for the classic secretary problem  (finding the maximum element) that achieves a competitive ratio  of $1-\epsilon$ (for any $\epsilon>0$)  using a shortlist of size $O(\log(1/\epsilon))$.
%for a class of submodular functions that we call them $m$-submodular,
%for any $m>0$. 
The algorithm  ignores an $\epsilon$-fraction of the input and then selects an item if it is greater than the maximum element seen so far. 
We show that with probability $1-\epsilon$, the total number of selections made by this algorithm is at most $O(\log (1/\epsilon))$.
%A special $m$-submodular function for $m=1$ is the function $\max$. 
%As a result we 
We will use this online algorithm as a subroutine in our proposed algorithm for \nameOfProblemSL, for repeatedly finding (with probability $1-\epsilon$) the  item with maximum marginal value with respect to a subset of items, under submodular function $f$.  %It requires $\log(1/\epsilon)$ selections.
The main idea of the algorithm for \nameOfProblemSL\ is to divide the input into some blocks that we call them $(\alpha,\beta)$ \textit{windows}.  In this procedure, we partition the input into slots, where the sizes of the slots follow a balls-and-bins distribution.  We then group these slots into windows.
%Divide the input into $k\beta$ slots. The $i$-th slot, $s_i$, consists of $X_i$ consecutive elements of the input.
%Random variables $\{X_i\}$  for $i\in [k\beta]$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha \beta$ consecutive slots.
%\begin{definition} 
%A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha$ consecutive intervals, 
%of length $n/k$. 
%each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
%Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%of length $\frac{n}{k\beta}$.
%\end{definition}
%It consists of $\alpha$ consecutive intervals, 
%%of length $n/k$. 
%each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
%Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%%of length $\frac{n}{k\beta}$.
%%Each window consists of smaller subintervals that we call them \textit{slots}.
Applying concentration inequalities for each {window}, and show that each window  has  roughly $\alpha$ elements of $OPT$ (the optimal solution), w.h.p.,
%the probability increases as $\alpha$ increases.
and that the fraction of elements of $OPT$ in a window that lie in different slots is at least $1-1/\beta$.
Therefore by choosing $\beta$ large enough most of the items in a window are in different slots, roughly speaking.\newline
For each window $w$ the algorithm \textit{guesses} the slots in which elements of $OPT$ in  $w$ lie in. 
By \text{guess} we mean that the algorithm enumerates over all subsets of size $\alpha$ of all $\alpha\beta$  slots in  $w$, and choose 
the one with the maximum marginal gain with respect to previously selected items. This can be done in an online manner.\newline
In the analysis of the algorithm for each window $w$,
we define an event $T_{1,\cdots, w-1}$ which conditions on the elements selected by the algorithm and also the positions in which they get selected by the algorithm. 
By conditioning on $T_{1,\cdots, w-1}$, we prove a lower bound for the expected marginal gain in the next window $w$.
Suppose $S_{1,\cdots, w-1}$ is output of the algorithm in windows $1,\cdots ,w-1$.
The crucial idea is that we show  conditioned on $T_{1,\cdots, w-1}$, each element $e\in OPT\setminus S_{1,\cdots, w-1}$
is more likely to appear in a slot in $w$ than in a slot in $1,\cdots, w-1$. 

We then have a normalization step in which we make all the elements of $OPT\setminus S_{1,\cdots, w-1}$ "appear" with the same probability in $w$. 
Therefore given that one slot in window $w$ contains an element of $OPT$, it can be any of $OPT\setminus S_{1,\cdots, w-1}$ with probability at least $1/k$. Hence the marginal gain for that slot is at least $\frac{1}{k}(OPT-F(S))$. 
We then repeat the argument for all the slots in window $w$  containing elements of the normalized sample.
\newline
The algorithm we describe uses $O(n)$ memory, in addition to the shortlist, but we can show how to modify the algorithm so that the amount of memory used is roughly the same as the size of the shortlist, and therefore the algorithm can be implemented in a streaming model.
} 

\subsection{Comparison to related work}
%There are two main frameworks  for \nameOfProblem: online algorithms and streaming algorithms.
%In the online framework,  we assume the input has random order. %(in adversarial order we can not guarantee anything)
%All of the previous algorithms in this framework irrevocably select a subset of size $k$, whose value is close to OPT~\cite{Bateni, kesselheim,Naor,smspm}.
We compare our results (Theorem \ref{opttheorem} and Theorem \ref{thm:streaming}) to the best known results for {\it \nameOfProblem}~and {\it \streamingProblem}, respectively.

The best known algorithm so far for \nameOfProblem~is by \citet{kesselheim}, with asymptotic competitive ratio of $1/e-O(k^{-1/2})$. 
In their algorithm, after observing each element, they use an oracle to compute optimal offline solution on the elements seen so far.
Therefore it requires exponential time in $n$. The best competitive ratio that they can get in polynomial time is 
$\frac{1}{e}(1-\frac{1}{e})-O(k^{-1/2})$.
In comparison, by using a shortlist of size $O(k)$ our (polynomial time) algorithm achieves a competitive ratio of $1-\frac{1}{e}-\epsilon-O(k^{-1})$. In addition to substantially improves the above-mentioned results for \nameOfProblem, this closely matches the best possible offline approximation ratio of $1-1/e$ in polynomial time. Further, our algorithm is linear time. Table \ref{table:t1} summarizes this comparison. 
Here, $O_\epsilon(\cdot)$ hides the dependence on the constant $\epsilon$. The hidden constant in $O_{\epsilon}(.)$ is %$c\frac{\log(1/\epsilon)}{\epsilon^2}  {\frac{1}{\epsilon^6} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^4} \log(1/\epsilon)}}$ 
\etaMacro for some absolute constant $c$.
%~\cite{Badanidiyuru2014StreamingFly} and~\cite{kesselheim}.

\begin{table}[h!]
\centering
\begin{tabular}{ |c c c c c| }
\hline
 & \#selections & Comp ratio & Running time & Comp ratio in poly(n) \\%&  Comp ratio in poly(n,k)  \\ 
\hline
\cite{kesselheim} & $k$ & $1/e-O(k^{-1/2})$ & $exp(n)$ & $\frac{1}{e}(1-1/e)$ \\ %& $(1-1/e)1/e$ \\ 
this & $O_{\epsilon}(k)$ & $1-1/e-\epsilon-O(1/k) $ & $O_{\epsilon}(n)$ &  $1-1/e-\epsilon-O(1/k)$ \\%&  $1-1/e-\epsilon$ \\
%2nd & $k\log^2 k$ & $1/2-O(k^{-1/4})$ & $poly(n), exp(k)$ & $1/2-O(k^{-1/4})$ & $(1/2-O(k^{-1/4}))(1-1/e)$ \\
\hline    

\end{tabular}
\caption{\nameOfProblem~settings}
\label{table:t1}
\end{table}
%On the other hand, in the streaming framework the decision to select an element is not irrevocable, and there is a buffer of limited size and you can add or remove elements from the buffer, i.e., you can deselect some elements that you have already selected. The random order assumption in this model is not necessary.
In the streaming setting, \citet{Chakrabarti2015} provided a single pass streaming algorithm for monotone submodular function maximization under $k$-cardinality constraint, that achieves a $0.25$ approximation under adversarial ordering of input. Further, their algorithm requires $O(1)$ function evaluations per arriving item and $O(k)$ memory.
The currently best known approximation  under  adversarial order streaming model is by~\citet{Badanidiyuru2014StreamingFly}, who achieve a $1/2-\epsilon$ approximation with a memory of size $O(\frac{1}{\epsilon}k\log k)$. 
%\scomment{no known? or is it not possible?}\mcomment{not possible}
%Any algorithm for streaming submodular
%maximization that only queries the value of the
%submodular function on feasible sets (i.e., sets of cardinality
%at most k) and is an α-approximation for a
%constant α > 0.5 must use Ω(n/k) memory, where n is
%the length of the stream.
There is an upper bound of $1/2+o(1)$ on the competitive ratio achievable by 
any algorithm for streaming submodular
maximization that only queries the value of the submodular function on feasible sets while using $o(n)$ memory~\cite{norouzi}.
%any streaming algorithm for this problem under adversarial order, while using $o(n)$ memory~\cite{norouzi}.
%It does not need random order assumption. 
%Also note that this algorithm can not be converted into an online algorithm. 
%Streaming algorithm with random order assumption has been considered for other problems. 
%But nothing better than~\cite{Badanidiyuru2014StreamingFly} is known for this problem under random order setting. 

\citet{Hess} initiated the study of  \streamingProblem.
Their algorithm uses $O(k)$ memory and a total of $n$ function evaluations to achieve $0.19$ approximation. 
%This result is  worse than the result of~\cite{kesselheim}  in the stricter online model. But note that~\cite{kesselheim} requires $\Omega(nk)$ function evalutation and $\Omega(n)$ memory.
The state of the art result in the random order input model is due to \citet{norouzi} who achieve a $1/2+8\times 10^{-14}$ approximation, while using a memory buffer of size $O(k\log k)$.
%Badanidiyuru et al.~\cite{Badanidiyuru2014StreamingFly} design the first efficient streaming algorithm
%with constant factor $1/2-\epsilon$ approximation guarantee, requiring only a single pass through the data, and memory $O(\frac{1}{\epsilon}k\log k )$.
%Recently~\cite{norouzi} showed that it is impossible to get ratio better than $1/2+o(1)$ in the adversarial order input using memory $o(n)$.
%Our algorithm is in the intersection of the above frameworks. 
%It generalizes the online framework in the way that we are allowed to select more than $k$ elements. 
%We generalize the online model in the way that we are allowed to select more than $k$ elements, and output a subset of size $k$ whose  value is close to OPT.  Note that we are only interested in returning a subset of size at most $k$ as our output.  
%In algorithms like ~\cite{Vondrak}, although the output is close to OPT, it is not restricted to $k$ elements, and we can't guarantee that it contains a subset of size $k$ whose value is close to OPT.
%In comparison, our algorithm selects $O(k)$ elements and guarantees that there is a subset of size $k$ whose value is $R-O(k^{-1})$ times $OPT$, for $R<1-1/e$.Thus by relaxing the number of selections we improve upon the best competitive ratio $1/e$, while only using $O(n)$ running time.  These bounds compare favorably to~\cite{kesselheim}, which  needs to find the optimal offline solution $n$ times, or to use an $1-1/e$ approximation to find each offline optimal solution. In the latter case, the running time is  $O(n^2)$ and the competitive ratio is  $\frac{1}{e} (1-1/e)$.
 
%It is asymptotically a $1/2-O(k^{-1/4})$ approximation algorithm.
%In terms of memory size, it improves upon the previous $k\log k$~\cite{norouzi}. %$\frac{1}{\epsilon}k\log k$.%, for $k>(1/\epsilon)^4$.
%(Note that the approximation ratio of our algorithm is asymptotic and for a fixed $k$ we can not decrease error more than $k^{-1/4}$)
%Also in terms of running time it is polynomial in $n$, but it requires exponential time in $k$.
%Also note that the online algorithm~\cite{kesselheim} can not be converted into a streaming algorithm with nontrivial memory size.

%The goal is to partition the items between agents so as to maximize the sum of their valuation functions.
%The well known greedy algorithm gives a 1/2 approximation for this problem. Also for the adversarial order 1/2 is the best we can achieve~\cite{Kapralov:2013}.
%\cite{vahab},~\cite{swm}  slightly improve the analysis of the greedy algorithm to just above 1/2 for  random order input (0.505, 0.509 competitive ratio respectively). The later result can be generalized to maximizing monotone sumobular functions subject to  a partition matroid. It is incomparable with \nameOfProblemSL.

%Table~\ref{table:t1} and 
Table~\ref{table:t2} provides a detailed comparison of our result in Theorem \ref{thm:streaming} to the 
%, we compare our algorithm to some of the previous works to show the tradeoffs in the various parameters for both the online algorithms model and the streaming model.
above-mentioned results for  \streamingProblem, showing that our algorithm substantially improves the existing results on most aspects of the problem. 

\begin{table}[h!]
\centering
\begin{tabular}{ |c c c c c | }
\hline
 & Memory size & Approximation ratio & Running time & update time \\ 
 \hline
\cite{Hess} & $O(k)$ &  $0.19$ & $O(n)$ & O(1) \\ 
\cite{norouzi} & $O(k\log k)$ &  $1/2+8\times 10^{-14}$ & $O(n\log k)$ & $O(\log k)$ \\ 
\cite{Badanidiyuru2014StreamingFly} & $O(\frac{1}{\epsilon}k\log k)$ & $1/2-\epsilon$ & $poly(n,k, 1/\epsilon)$ & $O(\frac{1}{\epsilon}\log k)$ \\ 
this & $O_{\epsilon}(k)$ & $1-1/e-\epsilon-O(1/k)$ & $O_{\epsilon}(n)$ & amortized $O_{\epsilon}(1+\frac{k^2}{n})$ \\
%2nd & $k\log^2 k$ & $1/2-O(k^{-1/4})$ & $poly(n), exp(k)$ &  \text{amortize one operation}\\
\hline    
\end{tabular}
\caption{\streamingProblem
}
%$\log(1/\epsilon) {\frac{1}{\epsilon^3} \log(1/\epsilon)  \choose {\frac{1}{\epsilon^2} \log(1/\epsilon)}}$.}
\label{table:t2}
\end{table}



There is also a line of work studying the online variant of the submodular welfare maximization problem (e.g., \cite{vahab,swm,Kapralov:2013}). In this problem, 
the items arrive online, and each arriving item should be allocated  to one of $m$ agents with a submodular valuation functions $w_i(S_i)$ where $S_i$ is the subset of items allocated to $i$-th agent). The goal is to partition the arriving items into $m$ sets to be allocated to $m$ agents, so that the sum of valuations over all agents is maximized. This setting is incomparable with the \nameOfProblem~setting considered here.

==> olderProof.tex <==
\begin{lemma}
\label{lem:piBound}
For any element $i\in S^*$, and $w \in \{1,\ldots, W\}$
\begin{equation}
p_i:=\mathbb{P}(i\in U_w \cup Supp(T_{1,\ldots, w-1}) | T_{1,\ldots, w-1}=T) \ge \frac{\alpha}{k}
\end{equation}
\end{lemma}
\begin{proof}
%Remember that from lemma~\ref{eqprob}, for every configuration $Y \in [k\beta]^n$, we have $\mathbb{P}(Y)=(k\beta)^{-n}$.
%Also from above lemma, for $1\le w\le W$,  $T_{1,\ldots, w}$ and $S_{1, \ldots, w}$ are uniquely defined for each configuration $Y$.
%Suppose $T_{1,\cdots, w-1}=T$ and 
Let $s$ be a slot in the first $w-1$ windows and $s'$ be a slot in window $w$.
If $i\in Supp(T)$ then the statement of the lemma is trivial, so suppose $i\notin Supp(T)$.
By applying Bayes' rule to equation~\ref{eq1} we have
\[
\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T) \frac{ \mathbb{P}(T_{1,\ldots, w-1}=T) }{\mathbb{P}(Y_i=s) } 
\le \mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) \frac{ \mathbb{P}(T_{1,\ldots, w-1}=T) }{\mathbb{P}(Y_i=s') } 
\]
Also from Lemma~\ref{indep}, $\mathbb{P}(Y_i=s)  = \mathbb{P}(Y_i=s')$ thus 
\[
\mathbb{P} (Y_i=s  | T_{1,\ldots, w-1}=T) 
\le \mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) 
\]
Furthermore, for slot $s"$ in  windows $w, w+1, \cdots, W$, by applying Bayes' rule to lemma~\ref{afterw}
we have $\mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) =\mathbb{P} (Y_i=s"  | T_{1,\ldots, w-1}=T)$.
As a result $\mathbb{P}(i \in U_w \cup R_{1,\ldots, w-1} | T_{1,\ldots, w-1}) \ge \frac{\alpha}{k}$.

\end{proof}
%And, for every  $i\in S^*$, define
%\begin{equation}
%p_i :=\mathbb{P}(i\in U_w \cup R_{1,\ldots, w-1} | T_{1,\ldots, w-1})
%\end{equation}
%Then, a corollary of Lemma \ref{lem:piBound} is that $p_i \ge \alpha/k$. 

\begin{lemma}
\label{JIN}
Fix a window $w$. Now, given $U_w, T_{1, \ldots, w-1}$, create $\tilde{S}$ by accepting each item $i\in S^* \cap (U_w \cup R_{1,\ldots, w-1})$ independently with probability $\alpha/(kp_i)$. Then,
the indicator random variables $\{{\mathbf 1}(i\in \tilde S)|T_{1,\ldots, w-1} \}$ for all $i\in S^*$ are independent with  expected value $\alpha/k$.
\end{lemma}
\begin{proof}
Using Lemma \ref{lem:piBound}, the expected value can be derived as
$$\mathbb{P}(i\in \tilde{S}| T_{1, \ldots, w-1}) = \mathbb{P}(i\in \tilde{S}| i\in U_w\cup R_{1,\ldots, w-1},T_{1, \ldots, w-1} )\mathbb{P}(i\in U_w\cup R_{1,\ldots, w-1}| T_{1, \ldots, w-1}) = \alpha/(kp_i) \times p_i = \alpha/k.$$
Next, we show that for any $i,j\in S^*$, random variables ${\mathbf 1}(i\in \tilde S)|T_{1,\ldots, w-1}$ and ${\mathbf 1}(j\in \tilde S)|T_{1,\ldots, w-1}$ are independent. Given the construction of $\tilde S$, it suffices to prove that the random variables ${\mathbf 1}(i\in U_w \cap R_{1,\ldots, w})|T_{1,\ldots, w-1}$ and ${\mathbf 1}(j\in U_w \cap R_{1,\ldots, w})|T_{1,\ldots, w-1}$ are independent. Now, given $T_{1,\ldots, w-1}=T$, if $i \in Supp(T)$ then this is trivial since $R_{1,\ldots, w} =Supp(T)$ so that $\mathbb{P}(i\in U_w \cap R_{1,\ldots, w} | T_{1,\ldots, w-1}=T)=1$. Similarly for $j\in Supp(T)$.

So, assume $i,j  \notin Supp(T)$. Then, the problem reduces to proving that  ${\mathbf 1}(i\in U_w)|T$ and ${\mathbf 1}(j\in U_w)|T$ are independent, i.e., given $T$, $i$ and $j$ will appear in the window $w$ independently. 
To prove this, we show that $\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T)=\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T \text{ and } Y_j =s')$, i.e., slot assignment of $i$ is independent of the slot assignment of $j$. 

Suppose $Y'$ is a configuration such that $Y'_i=s$ and $Y'_j=s'$, and $T_{1,\cdots, w-1}(Y')=T$. To show the required independence, we show that for every other feasible slot assignment of $j$, there exists a feasible configuration where slot assignment of $i$ is $s$.
More precisely, consider any configuration $Y''$ such that $T_{1,\cdots, w-1} (Y'') =T$ and $Y''_j=s''$ where $s''\ne s'$. (If no such configuration $Y''$ exists, then $Y_j|T$ is always $s'$ so that $s'$ is the only feasible assignment of $j$ given $T$, and the desired statement is trivially true.)
Then by changing $Y_j$ from $s'$ to $s''$ in $Y'$, we can obtain another configuration $\bar{Y}$. In Lemma~\ref{addtoslot}, we show that this change will not effect $T_{1,\cdots, w-1}$, i.e., $T_{1,\cdots, w-1} (\bar Y)=T $. 
Thus configuration $\bar Y$ satisfies the desired statement.
\end{proof}
\scomment{I replaced the proof below with the proof of Lemma 7}
\toRemove{
\begin{proof}
Suppose $i,j \in S^*$. 
If $i \in Supp(T) $ then this is trivial since $\mathbf{1}(i\in \tilde S) | T=1$. \scomment{the preceding statement is not correct, in that case, we just have $p_i=1$.}
So suppose $i,j  \notin Supp(T)$. 
%Now we show that $\mathbb{P}(J_i=1|T_{1,\cdots, w-1}=T)=\mathbb{P}(J_i=1|T_{1,\cdots, w-1}=T \text{ and } J_j =s')$.
Now we show that $\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T)=\mathbb{P}(Y_i=s|T_{1,\cdots, w-1}=T \text{ and } Y_j =s')$.
Suppose $Y$ is a configuration in which $Y_i=s$ and $Y_j=s'$, and $T_{1,\cdots, w-1} (Y)=T$.
Also suppose there exists at least one configuration $\bar{Y}$ such that $T_{1,\cdots, w-1} (\bar{Y}) =T$ and $\bar{Y}_j=s"$. \scomment{what if no such configuration exists?}
Then by changing $Y_j$ from $s'$ to $s"$ we obtain a configuration $Y'$. Also from lemma~\ref{addtoslot}, we have  $T_{1,\cdots, w-1} (Y')=T $. 
%It is because in configuration $Y$, $j$ has not been selected in slot $s'$ and its removal will not change $T_{1,\cdots, w-1}$.
%Furthermore since there is a configuration $\bar{Y}$ as described above, adding $j$ to $s"$ will not change $T_{1,\cdots, w-1}$.
Hence the mapping from $Y$ to $Y'$ proves lemma.
\end{proof}
}

\begin{lemma} \label{addtoslot}
Fix a slot $s'$, $T$, $j\notin Supp(T)$. Suppose that there exists  some configuration  $Y'$ such that $T_{1,\cdots, w-1} (Y') =T$ and $Y_j'=s'$. Then, given any configuration $Y''$ with $T_{1,\ldots, w-1}(Y'')=T$, we can replace  $Y''_j$ with $s'$ to obtain a new configuration $\bar Y$ that also satisfies $T_{1,\ldots, w-1}(\bar Y)=T$.
\toRemove{
Suppose there exists at least one configuration $\bar{Y}$ such that   $T_{1,\cdots, w-1} (\bar{Y}) =T$ and $\bar{Y}_j=s$ for $j\notin Supp(T)$.
Then for any configuration $Y$ with  $T_{1,\cdots, w-1} (Y) =T$, by setting $Y_j=s$, we get a new configuration $Y'$
such that $T_{1,\cdots, w-1} (Y') =T$.}
\end{lemma}
\begin{proof}
%Suppose $Y$ is a configuration such that $T_{1,\cdots, w-1} (Y) =T$. 
Suppose the slot $s'$ lies in window $w'$.
If $w' \ge w$ then the statement is trivial. So suppose $w' < w$.
Create an intermediate configuration by {\it removing} the item $j$ from $Y''$, call it $Y^-$. Since $j\notin Supp(T_{1,\cdots, w-1}(Y'')) = Supp(T)$ we have $T_{1,\cdots, w-1} (Y^-) =T$. In fact, for every subsequence $\tau$, the greedy subsequence for $Y''$, will be same as that for $Y^-$, i.e.,   $\gamma_{Y''}(\tau) = \gamma_{Y^-}(\tau)$.
Now add item $j$ to slot $s'$ in $Y^-$, to obtain configuration $\bar Y$. We claim $T_{1,\cdots, w-1} (\bar Y) =T$.
%We only need to show that $j$ will not get selected in slot $s$ in configuration $Y'$.
%Suppose not, then there is a subsequence $\tau$  in the algorithm ending in slot $s$ such that $\gamma_{Y'} (\tau) =\{i_1, \cdots, i_{t-1}, j\}$


By construction of $T_{1,\ldots, w}$, we only need to show that $j$ will not be part of the greedy subsequence $\gamma_{\bar Y}(\tau)$ for any subsequence $\tau, |\tau| = \alpha$ containing the slot $s'$ when the input is in configuration $\bar Y$. To prove by contradiction, suppose that $j$ is part of greedy subesquence for some $\tau$ ending in the slot $s'$. \toRemove{We only need to show that $j$ will not get selected in slot $s$ in configuration $Y'$.
Suppose $j$ gets selected in slot $s$ for some subsequence $\tau$ ending in slot $s$.}
%Thus $\gamma_{Y'}(\tau) = \{i_1, \cdots, i_{t-1}, j\}$. Note that since slots before $s$ are the same as $Y^-$ and $T_{1,\cdots, w-1} (Y^-) =T$, $\gamma_{Y^-}(\tau) = \{i_1, \cdots, i_{t-1}, i_t\}$.
\toRemove{Suppose that $\gamma_{Y^-}(\tau)  := \{i_1, \cdots, i_{t-1}, i_t\} = \gamma_{Y''}(\tau) $.} 
For this $\tau$, let $\gamma_{Y^-}(\tau)  := \{i_1, \cdots, i_{\alpha-1}, i_\alpha\} = \gamma_{Y''}(\tau) $. Note that since the items in the  slots  before $s'$ are identical for $\bar Y$ and $Y^-$, \toRemove{and $T_{1,\cdots, w-1} (Y^-) =T$,} we must have that $\gamma_{\bar Y}(\tau) = \{i_1, \cdots, i_{\alpha-1}, j\}$, i.e.,
$\Delta_f(j | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{\alpha-1}\} ) \ge \Delta_f(i_\alpha | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{\alpha-1}\} ) $.
%$j=\arg \max_{i\in j\cup U_s \cup T_{1, \ldots, w-1}} \Delta_f(i | S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{t-1}\} \cup \{i\}) $
%$i_t=\arg \max_{i\in U_s \cup T_{1, \ldots, w-1}} \Delta_f(i | S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{t-1}\} \cup \{i\}) $
On the other hand, since $T_{1,\cdots, w'-1} (Y') = T_{1, \cdots, w'-1}(Y'') = T (\text{restricted to $w'-1$ windows})$,  we have that $\gamma_{Y'} (\tau) =\{i_1, \cdots, i_\alpha\}$.
However, $Y'_j=s'$. Therefore $j$ was not part of the greedy subsequence $\gamma_{Y'}(\tau)$ even though it was in the last slot in $\tau$, implying $\Delta_f(j | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{t-1}\} ) < \Delta_f(i_t | S_{1,\ldots,w'-1} \cup \{i_1,\ldots, i_{t-1}\} ) $. This is  is a contradiction to the earlier observation.


\end{proof}
%Now let  indicator random variable $J_i$ for $i\in S^*$ indicates whether or not $i \in \tilde{S}$ 
%indicates whether or not $e$ appears in $U_w$, i.e., whether or not $U_i^e\in W_{i+1}$.



%Also if $V_e$ is a random variable indicating whether or not $e\in \mathcal{A}$ for $e\in OPT'$,
%we show $\{V_e|Snapshot(i)\}_{e\in OPT'}$ are i.i.d.  with $\mathbb{P}[V_e=1] = \alpha/k$.

%\begin{lemma}
 % %$\mathbb{P}[e=b_j| e\in \mathcal{A}]=1/k$ for $j\in[k]$.
% Random variables $\{V_e|Snapshot(i)\}$,  $ \forall e\in OPT'$ are i.i.d. with $\mathbb{P}[V_e=1]=\alpha/k$.
%\end{lemma}

%\begin{prop}\label{uni}
% Given $i \in \tilde{S}$, we have $\mathbb{P}(i=j)=1/k$, $\forall j\in S^*$.
%\end{prop}

%\scomment{The lemma statement below is not precise- it seems you actually mean uniformly at  random over $\tilde S|T_{1,\ldots, w-1}$, i.e., random also over $U_w$, but given $T_{1, \ldots, w-1}$. We can discuss.}
\begin{prop}\label{uni}
For element $i$ drawn uniformly at random from $\tilde{S}$, we have $\mathbb{P}(i=e)=1/k$, $\forall e\in S^*$.
\end{prop}




Now each element in $\tilde{S}\cap U_w$ has a unique slot in $w$. 
\begin{prop}
Suppose $p_1, \dots, p_{\ell}$ are the slots in $w$ containing at least one element of $\tilde{S}\cap U_w$ (in the same order that they appear in $w$). 
In addition, suppose $b_j\in p_j\cap \tilde{S}$, is the element of $\tilde{S}\cap U_w$ in slot $p_j$ (in case there are more than one element choose one randomly).
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
Then $b_1, \cdots, b_{\ell}$ is a random order of $\{b_1, \cdots, b_{\ell}\}$, and $\{b_1, \cdots, b_{\ell}\}$ are drawn uniformly at random from $\tilde{S}\cap U_w$.
\end{prop}
\scomment{Is Proposition 3 same as saying that $\{Y_i, i\in \tilde S\cap U_w\}$ are i.i.d. and uniformly distributed over slots in $w$? Where is the proof of this proposition?}
\mcomment{Yes, it follows from lemma 7 and the fact that we showed in lemma 6: for slot $s"$ in  windows $w$, by applying Bayes' rule to lemma~\ref{afterw}
we have $\mathbb{P} (Y_i=s'  | T_{1,\ldots, w-1}=T) =\mathbb{P} (Y_i=s"  | T_{1,\ldots, w-1}=T)$.}
%\begin{prop}\label{rord}
%%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
%$a_1, \cdots, a_t$ is a random order of $\{a_1, \cdots, a_t\}$, and $\{a_1, \cdots, a_t\}$ are drawn uniformly at random from $\tilde{S}$.
%\end{prop}

On the other hand, elements of $\tilde{S}\cap R_{1,\ldots, w-1}$ 
are not assigned to a  unique slot in $w$ (in the algorithm they were compared against the maximum marginal value in all the slots of $w$).
So we can assign each of them to a unique random slot in $w$.

\begin{prop}
Suppose $q_1, \dots, q_{m}$ are the slots in $w$ assigned to at least one element of $\tilde{S} \cap R_{1,\ldots, w-1}$ (in the same order that they appear in $w$). 
Furthermore, suppose $c_j\in q_j\cap \tilde{S}$, is the element of $\tilde{S}\cap R_{1,\ldots, w-1}$ in slot $q_j$ (in case there are more than one element choose one randomly).
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
Then $c_1, \cdots, c_m$ is a random order of $\{c_1, \cdots, c_m\}$, and $\{c_1, \cdots, c_m\}$ are drawn uniformly at random from $\tilde{S}\cap R_{1,\ldots, w-1} $.
\end{prop}


Now suppose $\{i_1, \cdots, i_t\}=\{p_1, \dots, p_{\ell}\} \cup \{q_1, \dots, q_{m}\}$ (in the same order that they appear in $w$).
From above propositions we have
\begin{prop}\label{rord}
Suppose $a_j \in i_j$  is an element of $i_j \cap (\{p_1, \dots, p_{\ell}\} \cup \{q_1, \dots, q_{m}\})$ (in case there are more than one element choose one randomly).Then
% $a_1, \cdots, a_m$ is a random order of $\{c_1, \cdots, c_m\}$, and $\{c_1, \cdots, c_m\}$ are drawn uniformly at random from $\tilde{S}\cap R_{1,\ldots, w-1} $.
%$a_1 ,\cdots, a_t$ are $t$ samples without replacement drawn uniformly at random from $\tilde{S}$.
$a_1, \cdots, a_t$ is a random order of $\{a_1, \cdots, a_t\}$, and $\{a_1, \cdots, a_t\}$ are drawn uniformly at random from $\tilde{S}$.
\end{prop}





%Consider the set $\mathcal{A}$ we create using the blackbox algorithm. It is a set that we create only for the purpose of argument. Algorithm~\ref{alg:khod} is not aware of this set. 
%Its existence is enough for the algorithm.
The algorithm \textit{guess} the position of elements of $\tilde{S}$, %$OPT\cap W_{i+1}$, 
i.e., slots $i_1, \cdots, i_t$. %, where $t \ge (1-\delta)\alpha$ w.h.p.
In other words, for some $\tau$ in the enumeration of algorithm,  the elements of $\tilde{S}$ lie in the slots of $\tau$. i.e., $\{i_1, \cdots, i_t\} \subseteq \tau$.
%Suppose $a_j\in i_j\cap \tilde{S}$, is the element of $\tilde{S}$ in slot $i_j$.
Suppose $s_j$ is the maximum element selected by the algorithm in $i_j$.
i.e., %$s_j=\omega(\{i_1,\dots,i_j\})$.
$s_j=argmax_{a\in i_j} \Delta_F(a| \gamma{(i_1,\ldots, i_{j-1})})$.
Also let's define $A(j)=\{a_1, \cdots, a_j\} $ and $S(w,j)= S_{1,\ldots, w-1} \cup \{s_1,\cdots, s_j\}$.

\begin{lemma}
%$\mathbb{E}[\Delta_F(S_w | S_{1,\ldots, w-1})] \ge \frac{t}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S_{1,\ldots, w-1})])$.
$\mathbb{E}[\Delta_F(s_{j+1}|S(w,j))] \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j))])$
\end{lemma}

\begin{proof}
\scomment{What is $OPT'$? What is $P$?}
\mcomment{$P:=S^*\setminus S_{1,\dots, w-1}$, Replaced}
From proposition~\ref{uni} and~\ref{rord}, $a_1$ can be any element in $S^*$, % $OPT\setminus P$, 
w.p. at least $1/k$.
Thus,
\[
\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1}) | T_{1,\ldots, w-1}] \ge \frac{1}{k} \sum_{e\in S^*} \Delta_F(e|S_{1,\ldots, w-1}) %=\frac{1}{k} \sum_{e\in OPT\setminus %P} \Delta_F(e|S_{1,\ldots, w-1}).
\]

%\[
%\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1}) | T_{1,\ldots, w-1}] \ge \frac{1}{k} \sum_{e\in OPT'} \Delta_F(e|S_{1,\ldots, w-1}) =\frac{1}{k} \sum_{e\in OPT\setminus P} \Delta_F(e|S_{1,\ldots, w-1}).
%\]
% (OPT-F(S(i)))$.


Now we use the following well known lemma:
\begin{lemma}%\label{marginalsum}
For any set $A$ and $B$, $\Delta_F(A|B) \le \sum_{a\in A\setminus B} \Delta_F(a|B)$
\end{lemma}
%(Note that in the original version of this lemma the sum is over $A$ instead of $A\setminus B$. But the above format is  stronger if  $A$ and $B$ have intersection. It is the reason we can assign value zero to dummy elements which represent the intersection).
Therefore,
\[
%OPT-F(S(i)) \le \sum_{e\in OPT} \Delta_F(e|S(i)) = \sum_{e\in OPT\setminus P} \Delta_F(e|S(i)) 
OPT-F(S_{1,\ldots, w-1}) \le  \sum_{e\in S^*}  %OPT\setminus P} 
\Delta_F(e|S_{1,\ldots, w-1})  %=  \sum_{e\in OPT'} \Delta_F(e|S(i)) 
\]
Hence,  
\[
\mathbb{E}[\Delta_F(a_1|S_{1,\ldots, w-1})|T_{1,\ldots, w-1}] \ge \frac{1}{k} (OPT-F(S_{1,\ldots, w-1})).
\]
%Now let's define $A(j)=\{a_1, \cdots, a_j\} $ and $S(w,j)= S_{1,\ldots, w-1} \cup \{s_1,\cdots, s_j\}$.
%denote $S(i)\cup \{s_1, \cdots, s_j\} $ by $S(i,j)$. 
Similarly, we can see that 
%$E[\Delta_F(a_{j+1}|S(i,j))] \ge \frac{1}{k} (OPT-F(S(i,j)))$.
\[
\mathbb{E}[\Delta_F(a_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] \ge  \frac{1}{k} \sum_{e\in S^*\setminus A(j)} \Delta_F(e|S(w,j)) 
%=\frac{1}{k} \sum_{e\in OPT\setminus (P\cup A(j))} \Delta_F(e|S(w,j)) 
%\ge \frac{1}{k} \sum_{e\in OPT\setminus (P\cup A)} \Delta_F(e|S(i,j))
\]
Also we have,
\begin{align*} %\label{eq1}
%\begin{split}
%A & = \frac{\pi r^2}{2} \\
% & = \frac{1}{2} \pi r^2
\sum_{e\in S^*\setminus A(j) } %OPT\setminus {(P\cup A(j))}} 
\mathbb{E}[\Delta_F(e|S(w,j)) | T_{1,\ldots, w-1}]  %= \sum_{e\in OPT\setminus P} \Delta_F(e|S(i,j)) 
&\ge \mathbb{E}[F(S^*\setminus A(j)) | T_{1,\ldots, w-1}]-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}] \\
&\ge \frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}] 
%\end{split}
\end{align*}
The last inequality coming from the fact that given $T_{1,\ldots, w-1}$, the set $A(j)$ is a random subset of $S^*$ of size at most  $\alpha$,
so we can apply the following lemma%~\ref{randomsubset}.
\begin{lemma}\label{randomsubset}
For a random subset $A$ of $R$, the expected value of $f(A)$ is at least $\frac{|A|}{k}.f(R)$.
\end{lemma}
Thus 
\[
\mathbb{E}[F(S^*\setminus A(j)) | T_{1,\ldots, w-1}] \ge \frac{k-\alpha}{k}OPT .
\]
Hence, 
\begin{align*}
\mathbb{E}[\Delta_F(s_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] &\ge \mathbb{E}[\Delta_F(a_{j+1}|S(w,j)) | T_{1,\ldots, w-1}] \\
& \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j)) | T_{1,\ldots, w-1}]) 
\end{align*}
Now by taking expectation over all possible realizations of $T_{1,\ldots, w-1}$,
\[
\mathbb{E}[\Delta_F(s_{j+1}|S(w,j))] \ge \frac{1}{k} (\frac{k-\alpha}{k}OPT-\mathbb{E}[F(S(w,j))])
\]
%Now by standard techniques we can deduce that $\mathbb{E}[F(S_{1,\ldots, W})] \ge (1-1/e)(\frac{k-\alpha}{k})(1-\delta) OPT$.

 \end{proof}

 
 
Now we prove 
elements of $\tilde{S}$ cover at least  $(1-\delta)\alpha$ slots in $w$, w.h.p. Let $t_w$  denote the number of these slots in $w$.

\begin{theorem}
%Elements of $\tilde{S}$ cover at least  $(1-\delta)\alpha$ slots in $w$, w.h.p.
$(1-\delta)\alpha \le t_w \le (1+\delta)\alpha$, w.h.p. 
\end{theorem}


%Therefore,
%$$\Ex[f(\tilde S \cup S_{1,\ldots, w-1}) - f(S_{1,\ldots, w-1})] \ge \frac{\alpha}{k} f(S^* \cup S_{1,\ldots, w-1}) - f(S_{1,\ldots, w-1}) $$
%INCOMPLETE: the expected size of $\tilde{S}$ is $\alpha$, but the realized size could be larger, and will be truncated to $\alpha$. We need to account for the decrease in objective due to this truncation.
By Chernouf bound, we can show that with high probability each window contains roughly $\alpha$ elements of $\tilde{S}$.

\begin{lemma}\label{bern}
%Suppose $W$ is a $(\alpha,\beta)$ window then
For window $w$
\[
\mathbb{P}(|\tilde{S}| < (1-\delta)\alpha ) %\le exp(-\frac{ (1/2)\alpha^{3/2}}{\alpha+1}) \le exp(-\sqrt{\alpha}/4)
\le \exp(-\delta^2 \alpha/2)
\]
\end{lemma}

Also we can show that roughly $\alpha-2\alpha/\beta$ slots in a window contain at least one element of $\tilde{S}$.

\begin{lemma}\label{slotlemma}
%The probability that one slot has two or more elements is at most $1-e^{-1/\beta}$.
%The fraction of nonempty slots with more than one elements of $OPT$ is at most $\beta(1-e^{1/\beta})$.
%The total number of slots  with more than one element of $OPT$  is at most $2\alpha/\beta$, w.h.p.
Given $|\tilde{S}|=r$,
the total number of slots in $W$ containing at least one element of $\tilde{S}$ is greater than %\alpha-2\alpha/\beta$  w.h.p.
$r(1-r/\alpha \beta)$  w.h.p.
%The total number of elements $e\in OPT\cap W$ such that $Y_e\cap OPT=\{e\}$ is at least $\alpha-2\alpha/\beta$.
%with more than one element of $OPT$  is at most $2\alpha/\beta$, w.h.p.
%$\beta(1-e^{1/\beta})$, w.h.p.
\end{lemma}
\begin{proof}

Suppose $\tilde{S}=\{a_1,\dots, a_r\}$.
%From previous lemma $r\le 2\alpha$, w.p. at least $1-\exp(-\sqrt{\alpha}/3)$.
Let $Z_i$ be a random variable indicating whether or not %$Y_{a_j}\cap OPT\neq \{a_j\}$.
$|Y_{a_j}\cap \{a_1,\dots, a_{j-1}\}| \ge 1$.
%indicating whether $a_k$ is alone in its slot or not.
We have at most $r$ occupied slots, thus the probability that $Z_i=1$ is at most $ r/(\alpha \beta) $ or $\mathbb{E}[Z_i]\le r/\alpha\beta$. Furthermore let $X_i=\sum_{j=1}^{i} Z_j$, then $\mathbb{E}[X_i] \le ri/\alpha\beta$.
%Also let $\mathcal{F}_i$ be the slots elements $1,\cdots, i$  are in, then $L\le \alpha/\beta$. 
Also define the set of filtration $\{\mathcal{F}_i\}$ to be the slots containing elements $\{a_1,\cdots, a_i\}$.
Then $\mathcal{F}_0 \subseteq \dots \subseteq \mathcal{F}_r$.
In addition, $L=\sum_{i\le r}  Var(Z_i|\mathcal{F}_{i-1}) \le r^2/\alpha\beta$.
By Freedman's inequality $\mathbb{P}( X_r > r^2/\alpha\beta + \epsilon )  \le exp(-\frac{\epsilon^2}{4r^2/\alpha\beta +2\epsilon})$.
\end{proof}

Suppose $\delta=1-1/e-R$.
From the above lemmas there are large enough constants $\alpha$ and $\beta$ such that:
\begin{itemize}
\item $r=|OPT\cap W| > (1-\delta/4)\alpha$. Thus $\alpha \ge \frac{1}{\delta^2} \log(1/\delta)$
\item The total number of slots in $W$ containing at least one element of $OPT$ is at least $(1-\delta)\alpha$.
Thus $(1-\delta/4)\alpha(1-(1-\delta/4)/\beta) > (1-\delta)\alpha$.
Therefore $\beta > (1-\delta/4)^2/(3/4\delta) $, so it suffices to have $\beta>\frac{4}{3\delta}$.
\end{itemize}
Hence we choose constants $(\alpha,\beta)$ with $\alpha \ge \frac{8}{\delta^2} \log(1/\delta)$ and $\beta>\frac{4}{3\delta}$,
so that we have above properties.

Therefore $\sum_{w} \min(\alpha, t_w) \ge (1-\delta)k$, w.h.p.
Now by standard techniques we can deduce that 
\begin{theorem}
$\mathbb{E}[F(S_{1,\ldots, W})] \ge (1-1/e)(\frac{k-\alpha}{k})(1-\delta) OPT$.
\end{theorem}

==> saved.tex <==
\noindent {\bf Offline algorithm}
We first present a simpler version of our algorithm which is easier to analyze but not implementable in an online manner. Then, in the next section, we will present an online algorithm which will mimic this offline algorithm very closely.

(Notation: We use shorthand $S_{1,\ldots, w}$ to denote $S_1\cup \cdots \cup S_{w}$.)

\begin{enumerate}
\item Initialize: constants $\alpha \ge 1, \beta \ge 1$ which depend on the constant $\epsilon$.
\item Divide input into $(\alpha, \beta)$ windows.
%Divide into windows and slots: Create $k/\alpha$ `windows'. Assign $n\alpha/k$ candidates to each window uniformly at random, let $U_w$ denote the set of candidates assigned to window $w$ for $w=1,\ldots, k/\alpha$. For each window $w$, create $\alpha\beta$ slots. Assign $\frac n {\beta k}$ out of $\frac {n \alpha} k$candidates to each slot uniformly at random, let $V_{j,w}$ denote the set of candidates assigned to slot $j$ in window $w$ for $j=1,\ldots, \alpha\beta$.
\item Initialize $S_0=\{\}, T_0=\{\}$.
\item For each window $w=1,\ldots, W$:
\begin{itemize}
\item For every $\alpha$-length subsequence $\tau=(s_1,\ldots, s_\alpha)$ of the $\alpha\beta$ slots in window $w$, find a `greedy' sequence $\gamma(\tau)$ of candidates, defined as:
$$\gamma(\tau):=\{i_1, \ldots, i_\alpha\}$$
where
$$i_j := \arg \max_{i\in V_{s_j,w} \cup R_{1,\ldots, w-1}} f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1\ldots, i_{j-1}\})$$
Note that $i_j$ can be picked either from the elements in slot $s_j$ or from $R_1\cup \cdots \cup R_{w-1}$.\\
({\bf To get the online version, primarily we need to use online max algorithm for this step})
\item Set $R_w$ as the union of all the greedy sequences above, i.e., 
$$R_w:=\{\cup_{\tau} \gamma(\tau)\}.$$ 
%where union is taken over all $\alpha$ length subsequences $\tau$ of slots in $w$.
\item Set $S_w$ as the `best' greedy sequence in $R_w$, i.e., $S_w=\gamma(\tau^*)$, where
$$\tau^*:=\arg \max_{\tau} f(S_{1,\ldots,w-1} \cup \gamma(\tau)) - f(S_{1,\ldots,w-1}).$$
\end{itemize}
\item Output $S_{1,\dots, W}$%$A=T_1 \cup \cdots  \cup T_{W}$
\end{enumerate} 
At the end of each window $w$, the above algorithm identifies a set of $\alpha$ `good' elements as the set $S_w$, which as we show later, will satisfy certain approximation properties compared to $\OPT- f(S_{1,\ldots, w-1})$. However, the algorithm actually picks a {\it larger set of elements} $T_w \supseteq R_w$. The set $R_w\backslash S_w$ acts as a buffer which can be used to pick some missed elements later as part of $S_{w'}$ for some window $w'>w$. 

%============================================================

\subsection{Overview and Techniques} 
First we design an asymptotic $1-\epsilon$ algorithm for finding maximum element in a random order input.
%a class of submodular functions that we call them $m$-submodular,
%for any $m>0$. 
The algorithm is very simple. 
It ignores the $\epsilon$-fraction of the input and then selects an item if it improves the current  solution.
We show that with probability $1-\epsilon$ the total number of selections is at most $\log (1/\epsilon)$.
%A special $m$-submodular function for $m=1$ is the function $\max$. 
%As a result we 
In our main algorithm for general monotone submodular functions we  will exploit the fact that we can find maximum marginal value 
of a given submodular function with respect to a subset of items with probability $1-\epsilon$ for $\epsilon>0$.  It requires $\log(1/\epsilon)$ selections.

The main idea of the algorithm is to divide the input into some blocks that we call them $(\alpha,\beta)$ \textit{windows}.
%\begin{definition}
 A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha$ consecutive intervals, 
%of length $n/k$. 
each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%of length $\frac{n}{k\beta}$.
%\end{definition}

%It consists of $\alpha$ consecutive intervals, 
%%of length $n/k$. 
%each interval is divided into $\beta$ slots. The length of $i$-th slot is a random variable denoted by $X_i$.
%Random variables $\{X_i\}$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
%%random sample from the binomial distribution $B(n,\frac{1}{k\beta})$.
%%of length $\frac{n}{k\beta}$.
%%Each window consists of smaller subintervals that we call them \textit{slots}.
We apply concentration inequalities for each \textit{window}, and first show that each window  has  roughly $\alpha$ elements of $OPT$, w.h.p., (the probability increases as $\alpha$ increases).
Then we show that the fraction of elements of $OPT$ in a window that lie in different slots is at least $1-1/\beta$.
Therefore by choosing $\beta$ large enough most of them are in different slots.

For each window $w$ the algorithm \textit{guess} the slots in which elements of $OPT\cap w$ lie in. 
By \text{guess} we mean that the algorithm enumerates over all subsets of size $\alpha$ of all $\alpha\beta$  slots in  $w$, and choose 
the one with the maximum marginal gain with respect to previously selected items. (this can be done in an online manner).

In the analysis of the algorithm for each window $w$,
we define an event $T_{1,\cdots, w-1}$ which conditions on the elements that are selected by the algorithm and also the positions in which they get selected by the algorithm. 
By conditioning on $T_{1,\cdots, w-1}$, we prove a lower bound for the expected marginal gain in  window $w$.
Suppose $S_{1,\cdots, w-1}$ is output of algorithm in the first $w$ windows.
The crucial idea is that we show  conditioned on $T_{1,\cdots, w-1}$, elements $e\in OPT\setminus S_{1,\cdots, w-1}$
are more likely to appear in a slot in $w$ than in a slot in windows $1, \cdots, w-1$. 

At the end we have a normalization step in which we make all the elements of $OPT\setminus S_{1,\cdots, w-1}$ to appear with the same probability in $w$. 
Therefore given that one slot in window $w$ contains an element of $OPT$, it can be any of $OPT\setminus S_{1,\cdots, w-1}$ with probability at least $1/k$. Hence the marginal gain for that slot is at least $\frac{1}{k}(OPT-F(S))$. 
We then repeat the argument for all the slots in window $w$  containing elements of the normalized sample.
%==========================================================

\subsection{Online version of the algorithm}

\noindent {\bf Online algorithm}
\begin{enumerate}
\item Initialize: constants $\alpha \ge 1, \beta \ge 1$ which depend on the constant $\epsilon$.
\item Divide into $(\alpha, \beta)$ windows.
%Divide the sequence of candidates into consecutive groups of $\frac{n}{\beta k}$ candidates, referred to as slots (or buckets). And, divide the sequence of slots into consecutive groups of $\alpha \beta$ slots, referred to as {\it windows}.
\item Initialize $S_0=\{\}, T_0=\{\}$.
\item For $w=1,\ldots, W=k/\alpha$:
\begin{itemize}
\item  for every slot $j$ in window $w$
\begin{itemize}
\item Concurrently for all subsequences $\tau\subseteq \{s_1, \ldots, s_{j-1}\}$ with $|\tau|<\alpha$ of slots in $w$, {\bf  run an online max algorithm} on the candidates in $s_j \cup R_{1, \ldots, w-1}$ to identify a set $I(j,\tau)\subseteq s_j \cup R_{1, \ldots, w-1}$ 
of at most  
$\log(1/\delta)$ elements such that the maximum marginal element:
%$$ i_j:=\arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} f(S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1,\ldots, i_{j-1}\})$$ 
$$ \arg \max_{i\in s_j \cup R_{1, \ldots, w-1}} f(S_{1,\ldots,w-1} \cup \gamma(\tau)\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \gamma(\tau)\})$$ 
lies in $I(j,\tau)$ with probability $1-\delta$. %$1-\frac{\delta}{\alpha{\alpha \beta \choose \alpha}}$. 
Here,
%$$\Gamma(\tau')= \{i_1, \ldots, i_{|\tau'|}\}$$
%with 

%$$i_j:= \max_{i\in I(j, \tau)} f(S_{1,\ldots,w-1} \cup \{i_1, \ldots, i_{j-1}\} \cup \{i\}) - f(S_{1,\ldots,w-1} \cup \{i_1, \ldots, i_{j-1}\})$$
\item {\bf Pick all the candidates in $I(j, \tau) \cap s_j$ for all $\tau$.}
\end{itemize}


\item Let $H_w$ be the union of all the (approximately) greedy sequences above, i.e., 
$$H_w:=\cup_{j\in w, |\tau|\le \alpha} (I(j,\tau)\cap s_j).$$ 
{\bf Note that at the end of window $w$, the candidates picked by the algorithm is $H_1 \cup \cdots \cup H_w$}.
%where union is taken over all $\alpha$ length subsequences $\tau$ of slots in $w$.

\item Set $R_w$ as the union of all the greedy 
%sequences $\tau\subseteq \{s_1, \cdots, s_{\alpha}\}$, i.e., 
$\alpha$-length subsequence $\tau=(s_1,\ldots, s_\alpha)$ of the $\alpha\beta$ slots in window $w$,
$$R_w:=\{\cup_{\tau} \gamma(\tau)\}.$$ 

%\item Set $S_w$ as the `best' subset of size $\alpha$ in $T_w$, i.e., 
%$$S_w:=\arg \max_{S\subseteq T_w, |S|\le \alpha} gf(S_{1,\ldots,w-1} \cup S) - f(S_{1,\ldots,w-1}).$$

\item Set $S_w$ as the `best' greedy sequence in $R_w$, i.e., $S_w=\gamma(\tau^*)$, where
$$\tau^*:=\arg \max_{\tau} f(S_{1,\ldots,w-1} \cup \gamma(\tau)) - f(S_{1,\ldots,w-1}).$$

\end{itemize}
\item Output $S_{1 \cup \cdots W} \cap H_{1,\cdots, W}$
%\item Output $T_1 \cup \cdots \cup T_{k/\alpha}$
\end{enumerate} 
%==========================================================
\subsection{$(\alpha,\beta)$-Windows}

\begin{definition}
Divide the input into $k\beta$ slots. The $i$-th slot, $s_i$, consists of $X_i$ consecutive elements of the input.
Random variables $\{X_i\}$  for $i\in [k\beta]$ are coming  from throwing $n$ balls into $k\beta$ bins, $X_i$ would be the number of balls in the $i$-th bin.
A \textit{window}, represented by parameters $(\alpha,\beta)$, consists of $\alpha \beta$ consecutive slots.
\end{definition}


Note that if the order of the input is $a_1, \dots, a_n$ then the elements inside $s_i$ are $a_{\ell}, a_{\ell+1}, \dots, a_{r}$
where $\ell=X_1+...+X_{i-1}+1$ and  $r=X_1+...+X_i$.





==> streaming.tex <==
\label{sec:streaming}
%\ccomment{Put here a short section explaining on how extend the algorithm to work for streaming.}
In this section, we show that Algorithm \ref{alg:main} can be implemented in a way that it uses a memory buffer of size at most $\eta(k)=O(k)$.
%also we compute the number of objective function evaluations for each arriving item as follows. 
% is $O(1+\frac{k^2}{n})$. %This will allow us to obtain  Theorem \ref{thm:streaming} (restated below) as a corollary of Theorem \ref{opttheorem}.
%\thmStreaming*
\toRemove{
\begin{restatable}{theorem}{thmStreaming}
\label{thm:streaming}
For any constant $\epsilon\in (0,1)$, there exists an algorithm for the \streamingProblem\ with matroid constraints  that achieves $\frac{1}{2}( 1-\frac{1}{e} -\epsilon -O(\frac{1}{k}))$ approximation to $\OPT$ while using a memory buffer of size at most $\eta_\epsilon(k)=O(k)$. Also, the number of objective  function evaluations for each item, amortized over $n$ items, is $O(pk+\frac{k^2}{n})$.
\end{restatable}
}
%Similar to matroid constraint 
For $p$-matchoid constraint we have the following result for the streaming setting. The proof appears in the appendix.\

%\thmStreamingMatchoid

\begin{restatable}{theorem}{thmStreamingMatchoid}
\label{thm:streamingMatcoid}
For any constant $\epsilon>0$, there exists an algorithm for the \streamingProblem\ with $p$-matchoid constraints  that achieves $\frac{1}{p+1}(1-\frac{1}{e^{p+1}} -\epsilon))$ approximation to $\OPT$ while using a memory buffer of size at most $\eta_\epsilon(k)=O(k)$. Also, the number of objective  function evaluations for each item, amortized over $n$ items, is $O(p\kappa+\kappa^p)$, where $\kappa= \max_{i\in[q]} rk(\mathcal{M}_i)$.
\end{restatable}
%\begin{proof}
%In the appendix.
%\end{proof}
\begin{proof}
The proof is similar to the one for matroid constraints, Theorem~\ref{thm:matroidstreaming}, which is omitted.
\end{proof}

\toRemove{
\begin{proof}
Th difference between Algorithm~\ref{alg:main} in this paper and the main Algorithm  in~\cite{us} is that, we remove elements of $\bar{S}_w$  from $S$ at the end of each window $w$. Therefore, with the same argument in the proof of Theorem 2 in~\cite{us}, we keep track of all parameters in Algorithm~\ref{alg:main} including $\bar{S}_w, S_w, R_w, \hat{S}_w$ in a memory efficient way using memory $O(k)$. 
The other difference between the two algorithms is in the subroutine~\ref{alg:matroidmax} that finds the element with maximum $g$ in a slot. 
In~\cite{us}, $g(e,S)$ can be computed using only one oracle access, whereas in the new definition of $g$ in equation~\ref{eq:newg}, we need access to independence oracle of $p$ matroids that $e$ belongs to, in order to check the independence of $S+e-e'$ for each $e' \in S$. At most $p \kappa$ elements of $S$ are eligible (they are in the ground set of a matroid that $e$ also member of). Hence, 
in order to create $\Omega_{\ell}(e,S)$, 
 for each arriving element $e$ in the input, we need $O(p\kappa)$ access to Independence oracle. Similarly the total access to the value oracle is $O(p\kappa)$. 
 In order to compute 
$\lambda(e,S)$, we need to consider all $\kappa^p$ combinations and have access to value oracle. Therefore the  number of access to the value oracle is $O(p\kappa+\kappa^p)$ per element. 
But, since the first element $a_0$ is computed in the beginning of each slot
for each $\tau$, we would have in average an additional $O(k^2/n)$ function evaluation per element.
\end{proof}
}

\toRemove{
\subsection{Max-Coverage}
One important monotone submodular function is max-coverage. 
\begin{definition} (max-coverage)
\end{definition}


Oracle access 

memory required to store each set.
}

% In the next section, we empirically compare our streaming algorithms with the state of the art algorithms in the streaming setting.
\toRemove{
In the current description of Algorithm \ref{alg:main}, there are several steps in which the algorithm potentially needs to store $O(n)$ previously seen items in order to compute the relevant quantities. 
%We discuss how to modify those steps to obtain an equivalent implementation but with memory buffer requirement of only $O(k)$. 
First, in Step \ref{li:subb}, in order to be able to compute $\gamma(\tau)$ for all less than $\alpha$ length subsequences $\tau$ of slots $s_1, \ldots, s_{j-1}$, the algorithm should have stored all the items that arrived in the slots $s_1, \ldots, s_{j-1}$. However, this memory requirement can be reduced by a small modification of the algorithm, so that at the end of iteration $j-1$, the algorithm has already computed  $\gamma(\tau)$ for all such $\tau$, and stored them to be used in iteration $j$. In fact, this can be implemented in a memory efficient manner, in the following way. For every subsequence $\tau$ of slots $s_1, \ldots, s_{j-1}$ of length $<\alpha$, consider prefix $\tau'=\tau\backslash s_{j-1}$. Assume $\gamma(\tau')$ is available from iteration $j-2$. 
If $\tau'=\tau$, then $\gamma(\tau)=\gamma(\tau')$. Otherwise, in Step 6 of iteration $j-1$, the algorithm must have considered the subsequence $\tau'$ while going through all subsequences of length less than $\alpha$ of slots $s_1, \ldots, s_{j-2}$. Now, modify the implementation of Step 6 so that  the algorithm also tracks the (true) maximum $M_{j-1}(\tau')$ of $a_0, a_1, \ldots, a_N$ for each $\tau'$. Then, $\gamma(\tau)$ can be obtained by extending $\gamma(\tau')$ by $M_{j-1}(\tau')$, i.e.,  $\gamma(\tau)=\{\gamma(\tau'), M_{j-1}(\tau')\}$. Thus, at the end of iteration $j-1$, $\gamma(\tau)$ would have been computed for all subsequences $\tau$ relevant for iteration $j$, and so on. In order to store these $\gamma(\tau)$ for every subsequence $\tau$ (of  at most $\alpha$ slots from $\alpha \beta$ slots), we require a memory buffer of size at most $\alpha^2{\alpha \beta \choose \alpha} = O(1)$.  

%In order to implement steps 6--9 for window $w$, and for every slot $s_j$, the algorithm needs a buffer to store $\tau, \gamma(\tau)$ for every subsequence  $\tau$ of length at most $\alpha$, of the $j-1$ slots in window $w$. This requires a memory buffer of size at most $\alpha \beta \times 2\alpha{\alpha \beta \choose \alpha}$. 
Secondly, across windows and slots, the algorithm keeps track of $R_w, S_w, w=1,\ldots, k/\alpha$ where $W=k/\alpha$. In the current description of Algorithm \ref{alg:main}, these sets are computed after seeing all the items in window $w$ in Step~\ref{li:Rw}. Thus, all the items arriving in that window would be needed to be stored in order to compute them, requiring $O(n)$ memory buffer. However, the alternate implementation discussed in the previous paragraph reduces this memory requirement to $O(k)$ as well. Using the above implementation, at the end of iteration $\alpha \beta$ for the last slot $s_{\alpha\beta}$ in window $w$, we would have computed and stored $\gamma(\tau)$ for all the subsequences  $\tau$ of length $\alpha$ of slots $s_1,\ldots, s_{\alpha\beta}$. 
$R_w$ is simply defined as union of all items in  $\gamma(\tau)$ over all such $\tau$ (refer to \eqref{eq:Rw}). And, $S_w = \gamma(\tau^*)$  for the best subsequence $\tau^*$ among these subsequences (refer to \eqref{eq:Sw}). 
Thus, computing $R_w$ and $S_w$ does not require any additional memory buffer. Storing $R_w$ and $S_w$ for all windows requires a buffer of size at most $\sum_w |R_w| + |S_w| = \frac{k}{\alpha} \times \alpha {\alpha \beta \choose \alpha}+ k = O(k).$
%Thus the subsequences considered in   to either add slot $s_j$. , by using the observation  that $R_w$ (as defined in \eqref{eq:Rw}) can be formed simply by adding all the union of all items in $A_j(\tau)$ The union of items these subsequences form $R_w$. Further, it needs to store $S_w$ for each window, which is of size $\alpha$. 
Therefore, the total buffer required to implement Algorithm \ref{alg:main} is of size $ O(k)$. 

%Finally, let's bound the number of objective function evaluations for each arriving item. Each arriving item is processed in Step 6, where objective function is evaluated twice for each $\tau$ to compute the corresponding $a_i$. Since there are atmost ${\alpha \beta \choose \alpha}$ subsequences $\tau$ for which this quantity is computed, the total number of objective function evaluations is  bounded by $2 {\alpha \beta \choose \alpha}=O(1)$. 
%This concludes the proof of Theorem \ref{thm:streaming}.

Finally, let's bound the number of objective function evaluations for each arriving item. Each arriving item is processed in Step 6, where objective function is evaluated twice for each $\tau$ to compute the corresponding $a_i$. Since there are atmost ${\alpha \beta \choose \alpha}$ subsequences $\tau$ for which this quantity is computed, the total number of times 
%the %Algorithm~\ref{alg:SIIImax} is called is 
%objective function evaluations is  
this computation is performed is bounded by $2 {\alpha \beta \choose \alpha}=O(1)$. However, for each $\tau$, we also compute $a_0$ in the beginning of the slot. Computing $a_0$ for each $\tau$ involves taking max over all items in $R_{1,\ldots, w-1}$, and requires $2|R_{1,\ldots,w-1}|\le 2k {\alpha \beta \choose \alpha}$ evaluations of the objective function. Due to this computation, in the worst-case, the update time for an item can be $ 2k {\alpha \beta \choose \alpha}^2 + 2 {\alpha \beta \choose \alpha}= O(k)$. However, since $a_0$ is computed {\it once} in the beginning of the slot for each $\tau$, the  total update time over all items is bounded by $2k {\alpha \beta \choose \alpha}^2 \times k\beta + {\alpha \beta \choose \alpha} \times n = O(k^2+n)$. Therefore the amortized update time for each item is $O(1+\frac{k^2}{n})$.
\scomment{replaced by above:Also each subroutine call on a slot $s_j$ goes over all elements in $s_j$ and also $R_{1,\cdots, w-1}$ to find the maximum element. 
%In the current format of the algorithm  
%The update time can be made to be at most $\frac{O(k^2)}{n}$ in this way. 
When we pass elements of $s_j\cup R_{1,\cdots, w-1}$ to the online subroutine~\ref{alg:SIIImax} one by one, for each element $e\in  s_j$ we can also pass $\frac{|R_{1,\cdots, w-1}|}{|s_j|}$ elements from $R_{1,\cdots, w-1}$. %Therefore, the expected update time for each element in $s_j$ would be  $\frac{O(k^2)}{n}$.
Therefore the amortized update time
would be $O(1+\frac{k^2}{n})$.
%in the beginning of each slot when we pass
Also note that the worst case update time can be $O(k)$.}
This concludes the proof of Theorem \ref{thm:streaming}.

Similarly for the $p$-matchoid constraints we have

%To conclude,  the following is obtained as a corollary of Theorem \ref{alg:main}.

%\noindent {\bf Theorem 2 (restated)}
%{\em For any constant $\epsilon>0$, there exists an algorithm for the \nameStreaming that uses a memory of size at most $\eta_\epsilon(k)=O(k)$, and achieves $1-\frac{1}{e} -\epsilon -O(\frac{1}{k})$ approximation to $\OPT$.
%Also it processes each arriving item with $O(1)$ evaluations
%of the objective function.}
}

%\subsection{Max-Coverage}

%\subsection{Max-Coverage}

%\subsection{Parallelization}


\mcomment{
\subsection{Experiment}
In this section, we consider uniform matroid, intersection of partition matroids and $p$-matchoid constraints. We compare our algorithm with state of the art algorithm for each type of constraint.
%using YouTube dataset and Twitter dataset described in the next section.
The experiments will be on Twitter stream summarization and YouTube Video
summarization tasks similar to the one in Kazemi et al.~\cite{kazemi2019submodular}.
Experiments for uniform matroids can be found in the Appendix.
}


\toRemove{
\subsubsection{DataSets}
The experiments will be on a Twitter stream summarization task and a YouTube Video
summarization task similar to the one in Kazemi et al.~\cite{kazemi2019submodular}.


\paragraph{\textbf{Twitter Stream Summarization}} In this application, we want to produce real-time summaries
for Twitter feeds. 
%Whether we want to provide a periodic synopsis of major
%events or simply to reduce the clutter in a user’s feed, 
%it would be very valuable if we could
It is valuable to create
a succinct summary that contains all the important information.
We use the dataset created by~\cite{kazemi2019submodular}.
They gather recent tweets from 30 different popular news accounts, to collect
a total of 42,104 unique tweets. 
They also define a monotone submodular function $f$ that covers the important stories of the day without
redundancy. It is defined as follows on a set $S\subseteq V$ of tweets:
$$
f(S):=\sum_{w\in W} \sqrt{\sum_{e \in S} score(w,e)}
$$

function f defined over a ground set $V$ of tweets. Each tweet $e\in V$ consists of a positive value
vale denoting its number of retweets and a set of $\ell_e$ keywords $W_e = \{w_{e,1}, \cdots, w_{e,\ell_e}\}$
from a general
set of keywords $W$. The score of a word $w\in W_e$ for a tweet $e$ is defined by $score(w, e) = vale_e$. If
$w\notin W_e$. Define $score(w, e) = 0$.


\paragraph{\textbf{YouTube Video Summarization}}
In this second task, we want to select representative frames
from video feeds.
We use the same data set as in~\cite{kazemi2019submodular}, which is YouTube videos of
New Year’s Eve celebrations from ten different cities around the world.

Using the first 30 seconds of each video, they train an autoencoder that compresses each frame into
a 4-dimensional representative vector. Given a ground set $V$ of such vectors,  define a matrix $M$
such that $M_{ij}=e-dist(v_i,v_j)$
, where $dist(v_i, v_j )$ is the euclidean distance between vectors 
$v_i, v_j \in V$.
Intuitively, $M_{ij}$ encodes the similarity between the frames represented by $v_i$ and $v_j$. 
They define a function as follows that intuitively measure the diversity of the
vectors in $S$:

The utility of a set $S\subseteq V$ is defined as a non-negative monotone submodular objective $f(S) =
\log det(I + \alpha M_S)$, where $I$ is the identity matrix, $\alpha > 0$ and $M_S$ is the principal sub-matrix of $M$
indexed by $S$. 

}

\toRemove{
\subsubsection{\textbf{Uniform Matroid}}
The simplest constraint that we can impose is the uniform matroid or equivalently the cardinality constraint.
In the simplest form our algorithm is similar to~\cite{us}.
We compare our algorithm to the state of the art algorithm in the streaming setting~\cite{kazemi2019submodular}.
%As we established an upper bound on the constant factor $\eta_{\epsilon}(k)$ in theorem~\ref{thm:streaming}, 
The performance of our algorithm crucially depends on the choice of 
$\alpha$ and $\beta$. The running time also is a function of $\alpha$ and $\beta$, and it grows rapidly as we increase $\alpha$ and $\beta$. 
Surprisingly, our algorithm outperforms~\cite{kazemi2019submodular}
%substantially 
even with relatively small choices of $\alpha=6$ and $\beta=2$.
We also observe that the utility of the output returned by our algorithm can be very  close to  what the optimal offline algorithm, namely the Greedy algorithm achieves. In Figure~\ref{fig:uniform}, we have plotted the performance of all three algorithms on the YouTube dataset.
Note that in our experiment we use a simplistic version of our algorithm in which we subsample from the shortlist in beginning of each window.
%and only use that subsample rather than the entire shortlist.
Furthermore we observe that our algorithm is slower than~\cite{kazemi2019submodular}, but the interesting fact about our algorithm 
%as stated in Theorem~\ref{thm:streaming} 
is that it is highly parallel, thus it has the potential to become $\eta_{\epsilon}(k)$  times faster.
%using parallelization. %(here roughly 1000 times).  
\begin{figure}[ht!]
\centering
\includegraphics[width=70mm]{correctFig.png}
\caption{The plot is for unifrom matroid, $\alpha =6$ and $\beta=2$}
\label{fig:uniform}
\end{figure}

}

%\subsubsection{$p$-matchoid constraints}
%\subsubsection{Intersection of Two Matroids}
\mcomment{
\subsubsection{\textbf{$p$-matchoid constraints}}
For the case of $p$-matchoid constraints, state of the art algorithm for general streaming setting is due to Feldman et al.~\cite{feldman2018streaming}.
In our experiment, we divide the elements of input into $q$ categories $\mathcal{N}= \mathcal{N}_1 \cup \cdots, \cup  \mathcal{N}_q$. 
We assign $p$ tags to each element $e$.
Each tag belongs to one of the categories $1,\cdots, q$ (generated randomly). 
Further, we impose a cardinality constraint $3$ for each category (i.e, $\mathcal{I}_{\ell} $ is a cardinality constraint).
The objective is to select at most $3$ elements from each category. In other words, an independent set of $p$-matchoid is defined as 
\[\mathcal{I}=\{S\subseteq \mathcal{N}: |S\cap \mathcal{N}_i|\le 3, \forall i\in [q] \}\]
In our algorithm, we  set $\alpha=3$ and $\beta=2$. We have plotted the performance of our algorithms and~\cite{feldman2018streaming} on the Twitter dataset below.
The first plot, Figure~\ref{fig:p3}, is for fixed $p=3$ and different number of categories $q$.
The second plot, Figure~\ref{fig:pmatchoid}, is for fixed number of categories $q=30$ and different values of $p$ from $1,\cdots, 10$. As the competitive ratio of our algorithm suggests, by  increasing $p$ the ratio of our utility versus the utility of~\cite{feldman2018streaming} increases.
%In order to create partitions we assign a label to each tweet, which represent the category it belongs to (generated randomly). We consider a $3$-matchoid constraint that is the intersection of a partition matroid with rank $k$.
%The goal is to choose at most 3 items from each partition.  We  set $\alpha=3$ and $\beta=2$. 
%We have plotted the performance of our algorithms and~\cite{feldman2018streaming} on the Twitter dataset below.
\begin{figure}[ht!]
\centering
%\includegraphics[width=100mm]{matroid.png}
\includegraphics[width=60mm]{tw3uni.png}
\caption{ The plot is for 3-matchoid constraint, and $\alpha =3$, $\beta=2$}
\label{fig:p3}
\end{figure}
\begin{figure}[ht!]
\centering
\includegraphics[width=60mm]{pmatchoidmany.png}
\caption{ The plot is for $p$-matchoid constraint, for $p=1,\cdots, 10$, and $\alpha =3$, $\beta=2$ and fixed $q=30$.}
\label{fig:pmatchoid}
\end{figure}
}
